Wavenumber-explicit stability and preasymptotic error analysis of UPML finite element method for obstacle scattering problems

This paper develops a wavenumber-explicit stability and preasymptotic error analysis for finite element approximation of the two-dimensional Helmholtz scattering problem with a uniaxial perfectly matched layer (UPML) truncation. The analysis is based on direct estimates of the stretched Green kernel associated with the Cartesian complex coordinate transformation. We establish explicit stability for the truncated UPML problem. In particular, we prove that the inf-sup constant of the truncated UPML formulation is $\mu_L = O(k^{-1})$ in a natural $k$-weighted $H^1$ norm. As a consequence, we also obtain an exponential decay estimate for the PML truncation error. Based on this stability estimate, we formulate a linear continuous interior penalty finite element method (CIP-FEM) on the truncated UPML domain. A key ingredient of the analysis is to establish a piecewise $H^{1+s}$-regularity result (for any $0<s<1$), which accounts for coefficient jumps across PML interfaces and singularities induced by Cartesian corner geometries. This fractional regularity is sufficient to derive wavenumber-explicit preasymptotic error estimates. Numerical experiments confirm the theoretical predictions and illustrate the effectiveness of the UPML CIP-FEM in the high-frequency regime.

==> est.tex <==

\section{Estimates of the modified Green's function}
\label{sec:kernel}

The purpose of this section is to deliver delicate estimates of the modified Green's function $\wt{G}$ and prove that $\wt{G}(\Bx,\By)$ decays exponentially as $|\Bx-\By|\to \infty$.


For a nonempty set $E\subset\bbR^2$ and a point $\Bx\in\bbR^2$, we define
\[
\mathrm{dist}_\infty(\Bx,E) :=\inf_{\Bz\in E}\|\Bx-\Bz\|_\infty, \quad
\|\Bx\|_\infty:=\max\{|x_1|,|x_2|\}.
\]
Write $a_+:=\max\{a,0\}$. If $\Bx\in B_l^c:=\bbR^2\backslash B_l$, it is easy to see that
\begin{align}\label{dist-Bl}
\mathrm{dist}_\infty(\Bx,B_l) =
\max\big\{ (|x_1|-l_1)_+,\ (|x_2|-l_2)_+ \big\}.    
\end{align}



\subsection{Estimates of $\Im\rho(\tilde\Bx,\tilde\By)$}
	

	
	\begin{remark}[Exponential far-field decay when $|\Bx-\By|\ge 2\sqrt2\,\beta l$]\label{rem:G-farfield-exp}
		Under the assumptions of Lemma~\ref{lem:Imrho-large-sep}, for all $\Bx\neq \By$ with
		$|\Bx-\By|\ge 2\sqrt2\,\beta l$,
		\begin{equation}\label{eq:G-farfield-exp}
			|G(\tilde{\Bx},\tilde{\By})|
			\le C\,(1+\sigma_0^2)^{1/4}\,
			\exp\!\Bigl(-\tfrac12 k\,c_\beta\sigma_0\,|\Bx-\By|\Bigr)\,
			(k|\Bx-\By|)^{-1/2},
		\end{equation}
		where \(c_\beta:=\frac12\frac{\beta-1}{\beta}\).
		Similarly, the derivative bounds in Lemma~\ref{lem:decay-stretchedG} gain the same exponential factor
		$\exp(-\tfrac12 k\,c_\beta\sigma_0\,|\Bx-\By|)$ in this far-field regime.
	\end{remark}

%%%

==> regularity-tmp.tex <==
\section{The CIP finite element method}
\label{sec:CIP-fem}

In this section, we prove a preasymptotic error estimate for the linear CIP-FEM approximation of the truncated PML problem \eqref{eq:weak-hu}. We shall adopt the duality technique developed in \cite{LiWu2019}. The key ingredients are the inf-sup condition \eqref{eq:infsup-OmL} and the piecewise fractional $H^{1+s}$-regularity (for any 
$0<s<1$) for elliptic equations with discontinuous UPML coefficients; the proof of the regularity result is provided in Appendix~\ref{app:sec:H1s-regularity}.


 

%We keep the notation for \(L^2\)-pairings from
%Section~\ref{sec:upml-prelim}.  In particular, no new inner-product notation is
%introduced in this section; sesquilinear pairings are written by inserting the
%complex conjugate in the second argument, for example \((f,\bar v)_\omega\).
%The bilinear form \(\mathscr A_\omega\) was defined in \eqref{a-R2}.  For the
%coercivity and duality arguments below we use the associated sesquilinear form
%\[
%        a_\omega(u,v)
%        :=
%        \mathscr A_\omega(u,\bar v)
%        =
%        \int_\omega
%        \left(
%        \bbA\nabla u\cdot\nabla\bar v
%        -
%        k^2Ju\bar v
%        \right),
%\]
%where
%\[
% \bbA=\operatorname{diag}(\alpha_2/\alpha_1,\alpha_1/\alpha_2),
%        \qquad
%        J=\alpha_1\alpha_2 .
%\]
%Thus the truncated UPML problem \eqref{eq:weak-hu} is equivalently written as:
%find \(\widehat u\in H^1_0(\Omega_L)\) such that
%\begin{equation}\label{eq:error1-continuous-problem}
%        a_{\Omega_L}(\widehat u,v)=(f,\bar v)_{\Omega_l}
%        \qquad\forall v\in H^1_0(\Omega_L).
%\end{equation}
%Here and below
%\[
%        \Omega_L=B_L\cap D^c,
%        \qquad
%        \Omega_l=B_l\cap D^c.
%\]


\subsection{Finite element space}
\label{sec:fem}

Let \(\Cp_L\) be the set of connected components of $B_L\backslash (\{x_1=\pm l_1\}\cup \{x_2=\pm l_2\})$. Each $Q\in\Cp_L$ is an open rectangle and $B_l\in\Cp_l$. The set of vertices of $\Cp_L$ is denoted by $\Cv_L$, which consists of four interior vertices at the corner of $B_l$ and twelve vertices on $\Gamma_L$. Then $\Cp_L$ induces a partition of $\Omega_L$ denoted by
\begin{align} \label{eq:PL}
\Cp_L^{\rm obs} = \big\{Q\cap \Omega_L: Q\in\Cp_L\big\}.
\end{align}





Let \(\widehat K\) be the reference triangle, and let $\mathcal T_h$ be a triangulation of $\ol\Omega_L$, which is fitted to \(\Gamma\), \(\Gamma_L\), and the UPML interfaces \(x_1=\pm l_1\) and \(x_2=\pm l_2\).  More precisely, each element \(K\in\mathcal T_h\) is closed and is the image of \(\widehat K\) under a \(C^2\)-diffeomorphism \(F_K\). 
The elements whose boundaries do not intersect $\Gamma$ are straight and their corresponding maps are affine, while the elements adjacent to \(\Gamma\) may be curved. For each $K\in\Ct_h$, $h_K$ denotes the diameter of $K$, and we assume
\[
\|D^mF_K\|_{L^\infty(\widehat K)}\le C h_K^m, \quad
\|D^mF_K^{-1}\|_{L^\infty(K)} \le C h_K^{-m}, \quad
m=1,2.
\]
Moreover, we assume $h:=\max\limits_{K'\in\Ct_h}h_{K'} \le C h_K$ for any $K\in\Ct_h$. Here the constants are independent of \(h\) and \(K\).  These assumptions are
standard for curved meshes (cf. \cite{Lenoir1986}).
The $H^1$-conforming finite element space is defined by pullback mappings
\[
V_h :=\big\{v_h\in H^1_0(\Omega_L):
v_h\circ F_K\in\mathbb P_1(\widehat K)
\quad\forall K\in\mathcal T_h\big\}.
\]

\subsection{Finite element approximation of \eqref{eq:weak-hu}}

For a domain $\Omega\subset\bbR^2$ and two real numbers $s,p>0$, we denote the conventional Sobolev norm and semi-norm on $W^{s,p}(\Omega)$ by $\N{\cdot}_{s,p,\Omega}$ and $\SN{\cdot}_{s,p,\Omega}$, respectively. For $p=2$, the conventional norm and semi-norm on $H^s(\Omega)$ are abbreviated to $\N{\cdot}_{s,\Omega}$ and $\SN{\cdot}_{s,\Omega}$, respectively. Define the broken Sobolev space 
\begin{align*}
H^s(\Cp_L^{\rm obs}) :=\,& \big\{v\in\Ltwo[\Omega_L]: \N{v}_{s,\Cp_L^{\rm obs}} < \infty\big\},  \\    
\|v\|_{s,\Cp_L^{\rm obs}}^2:=\,& \sum_{Q\in\mathcal P_L^{\rm obs}}\|v\|_{H^s(Q)}^2 , \quad  
|v|_{s,\Cp_L^{\rm obs}}^2:=
\sum_{Q\in\mathcal P_L^{\rm obs}}|v|_{H^s(Q)}^2 .
\end{align*}

Inspired by Li and Wu \cite{LiWu2019}, we shall penalize the numerical solution on edges inside $\Omega_l$, the set of which is denoted by $\Ce_h$. 
For \(E\in\Ce_h\), define $\omega_E:=\hbox{interior}(K^+\cup K^-)$ with $K^\pm\subset\Omega_l$ being the two elements sharing \(E\). Across $E$, the jump of normal derivative of a function $v$ is denoted by 
\[
\jump[E]{\partial_\Bn v} :=
\nabla \big(v|_{K^+}\big) \cdot \Bn 
-\nabla \big(v|_{K^-}\big)\cdot \Bn,
\]
where $\Bn$ denotes the unit normal of $E$. Define the interior penalty term by
\[
\mathscr{J}_h(u,v):=\sum_{E\in \Ce_h}\gamma_E h_E
\int_E\jump[E]{\partial_{\Bn}u}\,
\jump[E]{\partial_{\Bn}v}.
\]
The penalty parameters $\gamma_E$ satisfy
\begin{equation}\label{eq:gammaE}
|\gamma_E|\le C_\gamma,\quad
\Re\gamma_E\ge -\gamma_0,
\end{equation}
for two constant $C_\gamma,\gamma_0>0$ independent of $h$ and $k$. In practice, $\gamma_0$ is chosen sufficiently small.  
For $1<s \le 2$, we define the bilinear form on $\zbHone\cap H^{s}(\Cp^{\rm obs}_L)$ by
\[
\mathscr{A}_h(u,v):= \mathscr{A}_{\Omega_L}(u,v) + \mathscr{J}_h(u,v).
\]
The CIP-finite element approximation to \eqref{eq:weak-hu} is to find \(u_h\in V_h\) such that
\begin{equation}\label{eq:weakh}
\mathscr{A}_h(u_h,v_h)=(f,v_h)_{\Omega_L}
\quad\forall\, v_h\in V_h .
\end{equation}

 
By \eqref{eq:hu-model}, we have $\Delta\hat{u} = -f-k^2\hat{u}\in \Ltwo[\Omega_l]$. This implies $\jump[E]{\partial_\Bn\hat{u}}=0$ for all $E\in\Ce_h$. Therefore, 
\[
\mathscr{A}_h(\hat{u},v_h) = \mathscr{A}_{\Omega_L}(\hat{u},v_h) =(f,v_h)_{\Omega_L}
\quad\forall\, v_h\in V_h.
\]
This yields the Galerkin orthogonality 
\begin{align}\label{eq:Galerkin-orth}
\mathscr{A}_h(\hat{u}-u,v_h) =0
\quad\forall\, v_h\in V_h.
\end{align}

\subsection{Modified elliptic projection}

Following Li and Wu \cite{LiWu2019}, we introduce a modified elliptic projection operator which will play an important role in our error analysis. In the UPML case, error estimates for the modified elliptic projection rely greatly on the local $H^{1+s}$-regularity result.

First we define two bilinear forms 
\[
\mathscr{B}(u,v) :=
\int_{\Omega_L}\bbA\nabla u\cdot\nabla v, \quad 
\mathscr{B}_h(u,v):=\mathscr{B}(u,v)+\mathscr{J}_h(u,v),\quad .
\] 

\begin{definition}[Modified elliptic projections]
\label{def:elliptic-projections}
For \(z\in H^1_0(\Omega_L)\) for which the following expressions are well
defined, define \(\Pi_h^+z,\Pi_h^-z\in V_h\) by
\[
        b_h(\Pi_h^+z,v_h)=b(z,v_h)
        \qquad\forall v_h\in V_h,
\]
and
\[
        b_h(v_h,\Pi_h^-z)=b(v_h,z)
        \qquad\forall v_h\in V_h .
\]
\end{definition}

We shall use the seminorm
\[
        S_h(v)^2
        :=
        \sum_{e\in \Ce_h}
        |\gamma_e|h_e
        \|[\partial_{n_e}v]\|_{L^2(e)}^2
\]
and the discrete Helmholtz-CIP norm
\[
        \|v\|_{1,k,h}^2
        :=
        \|\nabla v\|_{L^2(\Omega_L)}^2
        +k^2\|v\|_{L^2(\Omega_L)}^2
        +S_h(v)^2 .
\]
For functions which are not finite element functions, \(S_h(v)\) is used only
when the normal derivative jumps on the edges of \(\Ce_h\) are well defined; in
particular, this is the case for functions which are locally \(H^2\) on the
penalized edge patches.


\begin{lemma}[Elliptic boundedness and coercivity]
\label{lem:Bh-stability}
Assume \eqref{eq:error1-penalty-assumption}.  If \(\gamma_0\) is sufficiently
small, then
\begin{equation}\label{eq:error1-Bh-bounded}
        |b_h(p,q)|
        \le
        C\bigl(\|\nabla p\|_{L^2(\Omega_L)}+S_h(p)\bigr)
         \bigl(\|\nabla q\|_{L^2(\Omega_L)}+S_h(q)\bigr),
\end{equation}
whenever the quantities are well defined.  Moreover, for every \(v_h\in V_h\),
\begin{equation}\label{eq:error1-Bh-coercive}
        \operatorname{Re} b_h(v_h,v_h)
        \ge c\|\nabla v_h\|_{L^2(\Omega_L)}^2,
\end{equation}
and
\begin{equation}\label{eq:error1-Sh-inverse}
        S_h(v_h)\le C\|\nabla v_h\|_{L^2(\Omega_L)} .
\end{equation}
The constants are independent of \(h\), \(k\), and \(v_h\).
\end{lemma}
\begin{proof}
The boundedness of the principal part follows from \(\bbA\in L^\infty\), and
\(|\mathscr{J}_h(p,q)|\le S_h(p)S_h(q)\) follows from Cauchy's inequality.  This proves
\eqref{eq:error1-Bh-bounded}.

For finite element functions, the mapped inverse trace inequality following from
the uniform assumptions on \(F_K\) gives
\[
        h_e\|[\partial_{n_e}v_h]\|_{L^2(e)}^2
        \le C\|\nabla v_h\|_{L^2(\omega_e)}^2 .
\]
Summing over \(e\in \Ce_h\) and using the finite overlap of the patches yields
\eqref{eq:error1-Sh-inverse}.

Since \(\alpha_j=1+i\sigma_j\) and \(0\le\sigma_j\le\sigma_0\),
\[
        \operatorname{Re}\frac{\alpha_2}{\alpha_1}
        =
        \frac{1+\sigma_1\sigma_2}{1+\sigma_1^2}
        \ge \frac1{1+\sigma_0^2},
        \qquad
        \operatorname{Re}\frac{\alpha_1}{\alpha_2}
        =
        \frac{1+\sigma_1\sigma_2}{1+\sigma_2^2}
        \ge \frac1{1+\sigma_0^2}.
\]
Therefore
\[
        \operatorname{Re}
        \int_{\Omega_L}\bbA\nabla v_h\cdot\nabla\overline{v_h}
        \ge a_0\|\nabla v_h\|_{L^2(\Omega_L)}^2
\]
for some \(a_0>0\) independent of \(h\) and \(k\).  On the other hand,
\[
        \operatorname{Re}\mathscr{J}_h(v_h,v_h)
        \ge
        -\gamma_0
        \sum_{e\in \Ce_h}h_e
        \|[\partial_{n_e}v_h]\|_{L^2(e)}^2
        \ge
        -C\gamma_0\|\nabla v_h\|_{L^2(\Omega_L)}^2 .
\]
Choosing \(\gamma_0\) sufficiently small proves \eqref{eq:error1-Bh-coercive}.
\end{proof}












\subsection{Piecewise $H^{1+s}$-regularity of the PML problem}


\begin{theorem}\label{thm:H1s-stability}
Assume the truncated UPML inf--sup estimate \eqref{eq:infsup-OmL}.  Since
\(v\mapsto\overline v\) is an isometry of \(H^1_0(\Omega_L)\), the same
inf--sup estimate holds for the sesquilinear form \(a_{\Omega_L}\).  Let
\(0<s<1\) be fixed.  If \(y\in H^1_0(\Omega_L)\) solves
\[
        a_{\Omega_L}(y,v)=(G,v)_{0,\Omega_L}
        \qquad\forall v\in H^1_0(\Omega_L),
\]
with \(G\in L^2(\Omega_L)\), then
\begin{equation}\label{app:eq:H1s-stability}
        |y|_{H^{1+s}(\mathcal P_L^{\rm obs})}
        \le
        C_s k\ln k\,\|G\|_{L^2(\Omega_L)} .
\end{equation}
The same estimate holds for the adjoint problem
\[
        a_{\Omega_L}(v,z)=(v,G)_{0,\Omega_L}
        \qquad\forall v\in H^1_0(\Omega_L).
\]
\end{theorem}

\begin{proof}
The estimate \eqref{eq:infsup-OmL}, written for the sesquilinear form
\(a_{\Omega_L}\), gives
\[
        \|y\|_{1,k,\Omega_L}
        \le
        Ck\ln k
        \sup_{0\ne v\in H^1_0(\Omega_L)}
        \frac{|(G,v)_{0,\Omega_L}|}{\|v\|_{1,k,\Omega_L}} .
\]
Since
\[
        |(G,v)_{0,\Omega_L}|
        \le
        \|G\|_{L^2(\Omega_L)}\|v\|_{L^2(\Omega_L)}
        \le
        k^{-1}\|G\|_{L^2(\Omega_L)}\|v\|_{1,k,\Omega_L},
\]
we have
\begin{equation}\label{app:eq:weighted-stability}
        \|y\|_{1,k,\Omega_L}
        \le
        C\ln k\,\|G\|_{L^2(\Omega_L)} .
\end{equation}
This implies
\[
        k^2\|y\|_{L^2(\Omega_L)}
        \le
        Ck\ln k\,\|G\|_{L^2(\Omega_L)} .
\]
Applying Theorem~\ref{app:thm:H1s-shift} and using \(J\in L^\infty(\Omega_L)\),
we obtain \eqref{app:eq:H1s-stability}.

For the adjoint problem, the direct estimate implies
\(\|T^{-1}\|\le Ck\ln k\), where \(T:H^1_0(\Omega_L)\to H^{-1}(\Omega_L)\) is the
operator induced by \(a_{\Omega_L}\) with the \(k\)-weighted norm.  Hence the
adjoint operator \(T^*\) satisfies the same inverse bound.  The preceding
argument, applied with \(\bbA^*\) and \(\overline J\), gives the adjoint
estimate.
\end{proof}



\begin{lemma}[Elementwise fractional Lagrange interpolation]
\label{lem:lagrange-fractional-interpolation}
Let \(0<s<1\) be fixed, and let
\[
        z\in H^1_0(\Omega_L)\cap H^{1+s}(\mathcal P_L^{\rm obs}).
\]
Let \(I_hz\) denote the mapped nodal Lagrange interpolant defined elementwise by
\[
        (I_hz)\circ F_K=\widehat I(z\circ F_K),
        \qquad K\in\mathcal T_h,
\]
where \(\widehat I\) is the nodal \(\mathbb P_1\) interpolant on the reference
triangle \(\widehat K\).  Then \(I_hz\in V_h\), and
\begin{equation}\label{eq:error1-lagrange-L2H1}
        \|z-I_hz\|_{L^2(\Omega_L)}
        +h\|\nabla(z-I_hz)\|_{L^2(\Omega_L)}
        \le
        C_s h^{1+s}\|z\|_{H^{1+s}(\mathcal P_L^{\rm obs})}.
\end{equation}
Moreover,
\begin{equation}\label{eq:error1-Sh-Ih}
        S_h(I_hz)
        \le
        C_s h^s |z|_{H^{1+s}(\mathcal P_L^{\rm obs})}.
\end{equation}
If, in addition, the normal derivative jumps of \(z\) on the penalized edges
are well defined and satisfy
\[
        [\partial_{n_e}z]=0,\qquad e\in \Ce_h,
\]
then
\begin{equation}\label{eq:error1-interpolation-edge}
        \|\nabla(z-I_hz)\|_{L^2(\Omega_L)}
        +S_h(z-I_hz)
        \le
        C_s h^s \|z\|_{H^{1+s}(\mathcal P_L^{\rm obs})}.
\end{equation}
\end{lemma}

\begin{proof}
We first explain why the mapped nodal interpolant is well defined.  Since the
mesh is fitted to \(\mathcal P_L^{\rm obs}\), every element \(K\in\mathcal T_h\)
is contained in the closure of one member of the partition.  Hence
\(z|_K\in H^{1+s}(K)\).  In two space dimensions, \(1+s>1=d/2\), and therefore
\(H^{1+s}(K)\hookrightarrow C^0(\overline K)\).  Thus all nodal values on each
element are meaningful.  If a node lies on a fitted interface between two
subdomains, the two continuous representatives give the same nodal value: indeed,
\(z\in H^1(\Omega_L)\) gives equality of the traces almost everywhere, and the
continuous representatives then agree everywhere on the edge.  Since
\(z\in H^1_0(\Omega_L)\), the boundary nodal values on
\(\Gamma\cup\Gamma_L\) are zero.  Consequently \(I_hz\in V_h\).

We next prove the interpolation estimate.  On a straight affine element \(K\),
the usual fractional nodal interpolation estimate gives
\begin{equation}\label{eq:error1-local-affine-lagrange}
        \|z-I_Kz\|_{L^2(K)}
        +h_K\|\nabla(z-I_Kz)\|_{L^2(K)}
        \le
        C_s h_K^{1+s}|z|_{H^{1+s}(K)} .
\end{equation}
This is the standard affine fractional Lagrange estimate; it follows from the
fractional Bramble--Hilbert lemma and the polynomial reproduction property of
the nodal \(P_1\) interpolant.  We cite
Sanchez--Arcangeli~\cite{SanchezArcangeli1984} for the fractional best
approximation and Lagrange interpolation estimates.

We now consider a curved boundary element \(K=F_K(\widehat K)\).  Put
\[
        \widehat z:=z\circ F_K,
        \qquad
        \widehat e:=\widehat z-\widehat I\widehat z .
\]
Then
\[
        (z-I_Kz)\circ F_K=\widehat e .
\]
On the fixed reference triangle, the nodal interpolation operator satisfies
\begin{equation}\label{eq:error1-reference-fractional}
        \|\widehat e\|_{H^1(\widehat K)}
        \le
        C_s |\widehat z|_{H^{1+s}(\widehat K)} .
\end{equation}
The constant depends on \(s\) and on the reference triangle, but not on \(K\).

We therefore need to estimate the fractional seminorm of the pullback
\(\widehat z=z\circ F_K\).  Since \(1+s\in(1,2)\),
\[
        |\widehat z|_{H^{1+s}(\widehat K)}
        \simeq
        |\widehat\nabla\widehat z|_{H^s(\widehat K)} .
\]
By the chain rule,
\[
        \widehat\nabla\widehat z
        =
        (DF_K)^T(\nabla z)\circ F_K .
\]
Let \(M:=DF_K\) and \(g:=(\nabla z)\circ F_K\).  For \(0<s<1\), the elementary
fractional product estimate on the fixed reference triangle gives
\[
        |M^Tg|_{H^s(\widehat K)}
        \le
        C_s\Bigl(
        \|M\|_{L^\infty(\widehat K)}|g|_{H^s(\widehat K)}
        +
        \|DM\|_{L^\infty(\widehat K)}\|g\|_{L^2(\widehat K)}
        \Bigr).
\]
Indeed, this follows directly from the Slobodeckij seminorm by writing
\[
M(\hat x)g(\hat x)-M(\hat y)g(\hat y)
=
M(\hat x)(g(\hat x)-g(\hat y))
+
(M(\hat x)-M(\hat y))g(\hat y),
\]
and using \(|M(\hat x)-M(\hat y)|\le \|DM\|_{L^\infty}|\hat x-\hat y|\);
the second double integral is finite because \(s<1\).

The mapped-element assumptions imply
\[
        \|M\|_{L^\infty(\widehat K)}\le Ch_K,
        \qquad
        \|DM\|_{L^\infty(\widehat K)}
        =
        \|D^2F_K\|_{L^\infty(\widehat K)}
        \le Ch_K^2 .
\]
The usual scaling relations under the uniformly regular map \(F_K\) give
\[
        |(\nabla z)\circ F_K|_{H^s(\widehat K)}
        \le
        C h_K^{s-1}|z|_{H^{1+s}(K)},
\]
and
\[
        \|(\nabla z)\circ F_K\|_{L^2(\widehat K)}
        \le
        C h_K^{-1}\|\nabla z\|_{L^2(K)} .
\]
Combining these estimates yields
\begin{equation}\label{eq:error1-pullback-H1s}
        |\widehat z|_{H^{1+s}(\widehat K)}
        \le
        C_s\left(
        h_K^s|z|_{H^{1+s}(K)}
        +
        h_K\|z\|_{H^1(K)}
        \right).
\end{equation}

Scaling \(\widehat e\) back to the physical element gives
\[
        \|z-I_Kz\|_{L^2(K)}
        +h_K\|\nabla(z-I_Kz)\|_{L^2(K)}
        \le
        C h_K\|\widehat e\|_{H^1(\widehat K)} .
\]
Together with \eqref{eq:error1-reference-fractional} and
\eqref{eq:error1-pullback-H1s}, this gives
\begin{equation}\label{eq:error1-local-curved-lagrange}
        \|z-I_Kz\|_{L^2(K)}
        +h_K\|\nabla(z-I_Kz)\|_{L^2(K)}
        \le
        C_s\left(
        h_K^{1+s}|z|_{H^{1+s}(K)}
        +
        h_K^2\|z\|_{H^1(K)}
        \right).
\end{equation}
Since \(0<s<1\) and \(h_K\le1\),
\[
        h_K^2\|z\|_{H^1(K)}
        \le
        h_K^{1+s}\|z\|_{H^{1+s}(K)} .
\]
Therefore \eqref{eq:error1-local-curved-lagrange} implies
\[
        \|z-I_Kz\|_{L^2(K)}
        +h_K\|\nabla(z-I_Kz)\|_{L^2(K)}
        \le
        C_s h_K^{1+s}\|z\|_{H^{1+s}(K)}
\]
on curved elements.

Combining this curved-element estimate with the affine estimate
\eqref{eq:error1-local-affine-lagrange}, summing over all elements, and using
the fittedness of the mesh with respect to \(\mathcal P_L^{\rm obs}\), we obtain
\eqref{eq:error1-lagrange-L2H1}.

It remains to estimate the penalty seminorm of \(I_hz\).  Let \(e\in \Ce_h\),
and let \(K^+\) and \(K^-\) be the two elements sharing \(e\).  By the definition
of \(\Ce_h\), the patch \(\omega_e=K^+\cup K^-\) is compactly contained in
\(\Omega_l\); in particular it does not meet \(\Gamma\), \(\Gamma_L\), or any
UPML coefficient interface.  Hence \(K^+\) and \(K^-\) are straight affine
elements.  Choose \(p_e\in\mathbb P_1(\omega_e)\).  Since affine functions have
no jump of the normal derivative across \(e\),
\[
        [\partial_{n_e}I_hz]
        =
        [\partial_{n_e}(I_hz-p_e)] .
\]
The inverse trace inequality on the two affine elements adjacent to \(e\) gives
\[
        h_e^{1/2}\|[\partial_{n_e}I_hz]\|_{L^2(e)}
        \le
        C\|\nabla(I_hz-p_e)\|_{L^2(\omega_e)} .
\]
Since \(I_hp_e=p_e\) on the affine patch,
\[
        \|\nabla(I_hz-p_e)\|_{L^2(\omega_e)}
        \le
        \|\nabla(z-p_e)\|_{L^2(\omega_e)}
        +
        \|\nabla((z-p_e)-I_h(z-p_e))\|_{L^2(\omega_e)} .
\]
The first term is bounded by the fractional best polynomial approximation
estimate on the affine patch \(\omega_e\), and the second term is bounded by
the affine interpolation estimate on \(K^+\) and \(K^-\).  Taking the infimum
over \(p_e\in\mathbb P_1(\omega_e)\), we obtain
\[
        h_e^{1/2}\|[\partial_{n_e}I_hz]\|_{L^2(e)}
        \le
        C_s h^s |z|_{H^{1+s}(\omega_e)} .
\]
Squaring and summing over \(e\in \Ce_h\), we find
\[
        S_h(I_hz)^2
        \le
        C_s h^{2s}\sum_{e\in \Ce_h}|z|_{H^{1+s}(\omega_e)}^2 .
\]
The patches \(\omega_e\) have uniformly finite overlap.  For the fractional part
of the seminorm, this follows because each pair \((x,y)\) belongs to only
uniformly finitely many products \(\omega_e\times\omega_e\).  Hence
\[
        \sum_{e\in \Ce_h}|z|_{H^{1+s}(\omega_e)}^2
        \le
        C |z|_{H^{1+s}(\mathcal P_L^{\rm obs})}^2 .
\]
This proves \eqref{eq:error1-Sh-Ih}.

If \([\partial_{n_e}z]=0\) on \(\Ce_h\), then
\[
        S_h(z-I_hz)=S_h(I_hz).
\]
Combining this identity with \eqref{eq:error1-lagrange-L2H1} and
\eqref{eq:error1-Sh-Ih} proves \eqref{eq:error1-interpolation-edge}.
\end{proof}

\begin{lemma}[Fractional projection estimates]
\label{lem:fractional-projection}
Let \(0<s<1\) be fixed.  Suppose that
\[
        z\in H^1_0(\Omega_L)\cap H^{1+s}(\mathcal P_L^{\rm obs})
\]
and that \([\partial_{n_e}z]=0\) on every edge \(e\in \Ce_h\).  Then
\(\Pi_h^\pm z\) are well defined and satisfy
\begin{equation}\label{eq:error1-proj-orth}
        b_h(z-\Pi_h^+z,v_h)=0,
        \qquad
        b_h(v_h,z-\Pi_h^-z)=0
        \qquad\forall v_h\in V_h .
\end{equation}
Moreover,
\begin{equation}\label{eq:error1-proj-H1}
        \|\nabla(z-\Pi_h^\pm z)\|_{L^2(\Omega_L)}
        +S_h(z-\Pi_h^\pm z)
        \le
        C_s h^s \|z\|_{H^{1+s}(\mathcal P_L^{\rm obs})},
\end{equation}
and, since \([\partial_{n_e}z]=0\) on \(\Ce_h\), this also implies
\begin{equation}\label{eq:error1-proj-Sh-Pi}
        S_h(\Pi_h^\pm z)
        \le
        C_s h^s \|z\|_{H^{1+s}(\mathcal P_L^{\rm obs})}.
\end{equation}
Finally,
\begin{equation}\label{eq:error1-proj-L2}
        \|z-\Pi_h^\pm z\|_{L^2(\Omega_L)}
        \le
        C_s h^{2s}\|z\|_{H^{1+s}(\mathcal P_L^{\rm obs})}.
\end{equation}
\end{lemma}

\begin{proof}
The well-posedness of the two projection problems follows from
Lemma~\ref{lem:Bh-stability}; for \(\Pi_h^-\) this is applied to the adjoint
elliptic form.  Since \(z\) has zero jumps on all penalized edges,
\[
        b_h(z,v_h)=b(z,v_h),
        \qquad
        b_h(v_h,z)=b(v_h,z),
\]
and the orthogonality relations \eqref{eq:error1-proj-orth} follow from the
definitions.

We prove \eqref{eq:error1-proj-H1} for \(\Pi_h^+\); the proof for
\(\Pi_h^-\) is identical with the arguments reversed.  Let
\[
        \delta_h:=\Pi_h^+z-I_hz\in V_h,
\]
where \(I_h\) is the mapped nodal Lagrange interpolant from
Lemma~\ref{lem:lagrange-fractional-interpolation}.  By coercivity,
orthogonality, and boundedness,
\[
        \|\nabla\delta_h\|_{L^2(\Omega_L)}^2
        \le
        C|b_h(\delta_h,\delta_h)|
        =
        C|b_h(z-I_hz,\delta_h)|
\]
\[
        \le
        C\bigl(\|\nabla(z-I_hz)\|_{L^2(\Omega_L)}+S_h(z-I_hz)\bigr)
        \|\nabla\delta_h\|_{L^2(\Omega_L)} .
\]
Using \eqref{eq:error1-interpolation-edge}, we obtain
\[
        \|\nabla\delta_h\|_{L^2(\Omega_L)}
        \le
        C_s h^s \|z\|_{H^{1+s}(\mathcal P_L^{\rm obs})} .
\]
Since
\[
        z-\Pi_h^+z=(z-I_hz)-\delta_h,
\]
the triangle inequality, \eqref{eq:error1-interpolation-edge}, and
\eqref{eq:error1-Sh-inverse} give \eqref{eq:error1-proj-H1}.  The estimate
\eqref{eq:error1-proj-Sh-Pi} follows from the identity
\(S_h(\Pi_h^\pm z)=S_h(z-\Pi_h^\pm z)\), which is a consequence of
\([\partial_{n_e}z]=0\) on \(\Ce_h\).

It remains to prove the \(L^2\)-estimate.  We again consider \(\Pi_h^+\) and set
\(e_\pi:=z-\Pi_h^+z\).  Let \(\phi\in H^1_0(\Omega_L)\) solve
\[
        b(v,\phi)=(v,\bar e_\pi)_{\Omega_L}
        \qquad\forall v\in H^1_0(\Omega_L).
\]
By Corollary~\ref{app:cor:H1s-stability} and the \(H^1\)-stability of the principal problem,
\[
        \|\phi\|_{H^{1+s}(\mathcal P_L^{\rm obs})}
        \le C_s\|e_\pi\|_{L^2(\Omega_L)},
        \qquad
        [\partial_{n_e}\phi]=0\quad(e\in \Ce_h).
\]
Therefore \(\mathscr{J}_h(e_\pi,\phi)=0\), and
\[
        \|e_\pi\|_{L^2(\Omega_L)}^2
        =b(e_\pi,\phi)
        =b_h(e_\pi,\phi).
\]
Using the projection orthogonality with \(I_h\phi\in V_h\),
\[
        \|e_\pi\|_{L^2(\Omega_L)}^2
        =b_h(e_\pi,\phi-I_h\phi).
\]
The boundedness of \(b_h\), \eqref{eq:error1-proj-H1},
\eqref{eq:error1-interpolation-edge}, and the preceding regularity estimate for
\(\phi\) imply
\[
        \|e_\pi\|_{L^2(\Omega_L)}^2
        \le
        C_s h^{2s}\|z\|_{H^{1+s}(\mathcal P_L^{\rm obs})}
        \|e_\pi\|_{L^2(\Omega_L)} .
\]
Dividing by \(\|e_\pi\|_{L^2(\Omega_L)}\), unless it is zero, proves
\eqref{eq:error1-proj-L2} for \(\Pi_h^+\).  The proof for \(\Pi_h^-\) uses the
principal dual problem
\[
        b(\psi,v)=(e_\pi,\bar v)_{\Omega_L}
        \qquad\forall v\in H^1_0(\Omega_L)
\]
and the second orthogonality relation in \eqref{eq:error1-proj-orth}.
\end{proof}

We shall use the following consequence of Corollary~\ref{app:cor:H1s-stability} and the continuous truncated UPML inf--sup estimate:
for every fixed \(0<s<1\),
\begin{equation}\label{eq:error1-uhat-H1s}
        \|\widehat u\|_{H^{1+s}(\mathcal P_L^{\rm obs})}
        \le
        C_s k\ln k\,\|f\|_{L^2(\Omega_l)} .
\end{equation}
Furthermore, if \(z_g\in H^1_0(\Omega_L)\) is defined by
\begin{equation}\label{eq:error1-adjoint-zg}
        a_{\Omega_L}(v,z_g)=(v,\bar g)_{\Omega_L}
        \qquad\forall v\in H^1_0(\Omega_L),
\end{equation}
then
\begin{equation}\label{eq:error1-zg-H1s}
        \|z_g\|_{H^{1+s}(\mathcal P_L^{\rm obs})}
        \le
        C_s k\ln k\,\|g\|_{L^2(\Omega_L)} .
\end{equation}

\begin{theorem}[Fractional preasymptotic CIP-FEM error estimate]
\label{thm:fractional-cip-error}
Assume that \(\Gamma\) is \(C^{\infty}\), \(D\Subset B_l\), that the mapped
fitted meshes satisfy the uniform assumptions stated above, that the PML
parameters are such that the truncated inf--sup estimate
\eqref{eq:infsup-OmL} holds, and that \eqref{eq:error1-penalty-assumption}
holds with \(\gamma_0\) sufficiently small.  Let \(0<s<1\) be fixed.  There
exist constants \(C_s>0\) and \(c_s>0\), independent of \(h\), \(k\), and \(f\),
such that, if
\begin{equation}\label{eq:error1-resolution-condition}
        k^3h^{2s}\ln k\le c_s,
\end{equation}
then the discrete problem \eqref{eq:error1-cip-method} has a unique solution
\(u_h\in V_h\).  Moreover,
\begin{equation}\label{eq:error1-L2-final}
        \|\widehat u-u_h\|_{L^2(\Omega_L)}
        \le
        C_s k^2h^{2s}(\ln k)^2
        \|f\|_{L^2(\Omega_l)},
\end{equation}
and
\begin{equation}\label{eq:error1-H1kh-final}
        \|\widehat u-u_h\|_{1,k,h}
        \le
        C_s\left(kh^s\ln k+k^3h^{2s}(\ln k)^2\right)
        \|f\|_{L^2(\Omega_l)} .
\end{equation}
\end{theorem}

\begin{proof}
We first derive the estimates for any discrete solution.  Let
\[
        e:=\widehat u-u_h .
\]
By Lemma~\ref{lem:penalty-consistency}, \(\mathscr{J}_h(\widehat u,v_h)=0\) for every
\(v_h\in V_h\).  Subtracting \eqref{eq:error1-cip-method} from
\eqref{eq:error1-continuous-problem} gives
\begin{equation}\label{eq:error1-Galerkin-orthogonality}
        a_h(e,v_h)=0
        \qquad\forall v_h\in V_h .
\end{equation}

We first prove the \(L^2\)-estimate.  Let \(z\in H^1_0(\Omega_L)\) solve
\begin{equation}\label{eq:error1-adjoint-for-e}
        a_{\Omega_L}(v,z)=(v,\bar e)_{\Omega_L}
        \qquad\forall v\in H^1_0(\Omega_L).
\end{equation}
Then \eqref{eq:error1-zg-H1s} gives
\begin{equation}\label{eq:error1-z-H1s}
        \|z\|_{H^{1+s}(\mathcal P_L^{\rm obs})}
        \le
        C_s k\ln k\,\|e\|_{L^2(\Omega_L)} .
\end{equation}
Moreover, Lemma~\ref{lem:penalty-consistency} gives zero normal derivative jumps
of \(z\) on all penalized edges.  Hence \(\mathscr{J}_h(e,z)=0\), and
\[
        \|e\|_{L^2(\Omega_L)}^2
        =a_{\Omega_L}(e,z)
        =a_h(e,z).
\]
Using \eqref{eq:error1-Galerkin-orthogonality} with \(\Pi_h^-z\in V_h\),
\begin{equation}\label{eq:error1-duality-start}
        \|e\|_{L^2(\Omega_L)}^2
        =a_h(e,z-\Pi_h^-z).
\end{equation}
Expanding \(a_h\) yields
\begin{equation}\label{eq:error1-duality-expand}
        \|e\|_{L^2(\Omega_L)}^2
        =
        b_h(e,z-\Pi_h^-z)
        -k^2(Je,\overline{z-\Pi_h^-z})_{\Omega_L}.
\end{equation}

For the principal part, decompose
\[
        e=(\widehat u-I_h\widehat u)+(I_h\widehat u-u_h).
\]
Since \(I_h\widehat u-u_h\in V_h\) and
\(b_h(v_h,z-\Pi_h^-z)=0\) for all \(v_h\in V_h\),
\[
        b_h(e,z-\Pi_h^-z)
        =
        b_h(\widehat u-I_h\widehat u,z-\Pi_h^-z).
\]
By \eqref{eq:error1-Bh-bounded}, \eqref{eq:error1-interpolation-edge},
\eqref{eq:error1-proj-H1}, \eqref{eq:error1-uhat-H1s}, and
\eqref{eq:error1-z-H1s},
\begin{equation}\label{eq:error1-principal-bound}
        |b_h(e,z-\Pi_h^-z)|
        \le
        C_s k^2h^{2s}(\ln k)^2
        \|f\|_{L^2(\Omega_l)}
        \|e\|_{L^2(\Omega_L)} .
\end{equation}
For the mass term, the boundedness of \(J\), \eqref{eq:error1-proj-L2}, and
\eqref{eq:error1-z-H1s} give
\begin{equation}\label{eq:error1-mass-bound}
\begin{aligned}
        k^2|(Je,\overline{z-\Pi_h^-z})_{\Omega_L}|
        &\le
        Ck^2\|e\|_{L^2(\Omega_L)}
        \|z-\Pi_h^-z\|_{L^2(\Omega_L)}  \\
        &\le
        C_s k^3h^{2s}\ln k
        \|e\|_{L^2(\Omega_L)}^2 .
\end{aligned}
\end{equation}
Combining \eqref{eq:error1-duality-expand}--\eqref{eq:error1-mass-bound}, we
obtain
\[
        \|e\|_{L^2(\Omega_L)}^2
        \le
        C_s k^2h^{2s}(\ln k)^2
        \|f\|_{L^2(\Omega_l)}\|e\|_{L^2(\Omega_L)}
        +
        C_s k^3h^{2s}\ln k\|e\|_{L^2(\Omega_L)}^2 .
\]
Choosing \(c_s\) in \eqref{eq:error1-resolution-condition} sufficiently small,
the last term is absorbed into the left-hand side.  This proves
\eqref{eq:error1-L2-final}.

We next prove the \(\|\cdot\|_{1,k,h}\)-estimate.  Define
\[
        \rho:=\widehat u-\Pi_h^+\widehat u,
        \qquad
        \eta:=u_h-\Pi_h^+\widehat u .
\]
Then \(e=\rho-\eta\).  By Lemma~\ref{lem:fractional-projection} and
\eqref{eq:error1-uhat-H1s},
\begin{equation}\label{eq:error1-rho-1kh}
        \|\rho\|_{1,k,h}
        \le
        C_s\bigl(kh^s\ln k+k^2h^{2s}\ln k\bigr)
        \|f\|_{L^2(\Omega_l)} .
\end{equation}
Since \(k\ge2\), the second term is bounded by the pollution-scale term after
enlarging \(C_s\):
\begin{equation}\label{eq:error1-rho-final}
        \|\rho\|_{1,k,h}
        \le
        C_s\left(kh^s\ln k+k^3h^{2s}(\ln k)^2\right)
        \|f\|_{L^2(\Omega_l)} .
\end{equation}
It remains to estimate \(\eta\).  Since \(\eta\in V_h\),
\eqref{eq:error1-Galerkin-orthogonality} gives \(a_h(e,\eta)=0\).  Using
\(e=\rho-\eta\), we get
\[
        0=b_h(\rho-\eta,\eta)-k^2(Je,\bar\eta)_{\Omega_L}.
\]
The \(\Pi_h^+\)-orthogonality gives \(b_h(\rho,\eta)=0\).  Hence
\begin{equation}\label{eq:error1-eta-identity}
        b_h(\eta,\eta)=-k^2(Je,\bar\eta)_{\Omega_L} .
\end{equation}
By Lemma~\ref{lem:Bh-stability},
\begin{equation}\label{eq:error1-eta-grad-bound-start}
        \|\nabla\eta\|_{L^2(\Omega_L)}^2+S_h(\eta)^2
        \le
        C|b_h(\eta,\eta)|
        \le
        Ck^2\|e\|_{L^2(\Omega_L)}\|\eta\|_{L^2(\Omega_L)} .
\end{equation}
Moreover, \(\eta=\rho-e\).  The projection estimate, \eqref{eq:error1-uhat-H1s},
and \eqref{eq:error1-L2-final} imply
\begin{equation}\label{eq:error1-eta-L2}
        \|\eta\|_{L^2(\Omega_L)}
        \le
        C_s k^2h^{2s}(\ln k)^2
        \|f\|_{L^2(\Omega_l)} .
\end{equation}
Substituting \eqref{eq:error1-L2-final} and \eqref{eq:error1-eta-L2} into
\eqref{eq:error1-eta-grad-bound-start}, we obtain
\[
        \|\nabla\eta\|_{L^2(\Omega_L)}+S_h(\eta)
        \le
        C_s k^3h^{2s}(\ln k)^2
        \|f\|_{L^2(\Omega_l)} .
\]
The same \(L^2\)-bound gives
\[
        k\|\eta\|_{L^2(\Omega_L)}
        \le
        C_s k^3h^{2s}(\ln k)^2
        \|f\|_{L^2(\Omega_l)} .
\]
Thus
\begin{equation}\label{eq:error1-eta-1kh}
        \|\eta\|_{1,k,h}
        \le
        C_s k^3h^{2s}(\ln k)^2
        \|f\|_{L^2(\Omega_l)} .
\end{equation}
Finally, \(e=\rho-\eta\), \eqref{eq:error1-rho-final}, and
\eqref{eq:error1-eta-1kh} prove \eqref{eq:error1-H1kh-final}.

It remains to show unique solvability.  Let \(f=0\), and let
\(u_h\in V_h\) be a solution of the homogeneous discrete problem.  Then the
continuous solution is \(\widehat u=0\).  Since the preceding \(L^2\)-estimate
was derived for any discrete solution, it gives
\[
        \|u_h\|_{L^2(\Omega_L)}
        =
        \|\widehat u-u_h\|_{L^2(\Omega_L)}
        \le
        C_s k^2h^{2s}(\ln k)^2\|f\|_{L^2(\Omega_l)}
        =0.
\]
Hence \(u_h=0\).  Thus the homogeneous discrete system has only the trivial
solution. The proof is finished.
\end{proof}

\begin{remark}[Relation with the total PML error]
Theorem~\ref{thm:fractional-cip-error} estimates the finite element error for
the truncated UPML solution \(\widehat u\).  Combining
\eqref{eq:error1-L2-final}--\eqref{eq:error1-H1kh-final} with the exponential
truncation estimate in Section~\ref{sec:obstacle} yields the corresponding error
estimate for the stretched exact solution \(\widetilde u\) by the triangle
inequality.
\end{remark}

\begin{remark}[Exact fitted geometry and polygonal computations]
The estimate in Theorem~\ref{thm:fractional-cip-error} is proved on the exact
truncated domain
\[
        \Omega_L=B_L\setminus\overline D
\]
with the fitted mapped finite element space defined above.  If, in a numerical
implementation, the smooth obstacle \(D\) is replaced by a polygonal obstacle
\(D_h\), then the computation is posed on
\[
        \Omega_{L,h}=B_L\setminus\overline{D_h},
\]
not on \(\Omega_L\).  In that case the observed numerical error contains both
the finite element error on the discrete domain and a geometry error caused by
the replacement of \(D\) by \(D_h\).  This geometry error is not quantified by
Theorem~\ref{thm:fractional-cip-error}.
\end{remark}

==> regularity.tex <==

\section{Regularity estimate for the UPML problem}
\label{app:sec:H1s-regularity}

The purpose of this appendix is to prove the piecewise $H^{1+s}$-regularity in Section~\ref{sec:fem}. Let $\Cp_L$, $\Cp_L^{\rm obs}$, and $\Cv_L$ be the partition of $B_L$, the partition of $\Omega_L$, and the set of vertices, respectively, which are defined in section~\ref{sec:fem}. 




%Let $\bbA$ and $J$ be the PML coefficients given in \eqref{eq:A-J} and let $\bbA^* = \bar\bbA^T$ be the conjugate transpose of $\bbA$. Both of them are discontinuous across interior boundaries of $\Cp_L$. 

We first record the local pencil property of the PML coefficients. Near a vertex of the partition, the possible corner singularities of an elliptic transmission problem are generated by the homogeneous principal
problem with zero boundary and interface data. The right-hand side and the lower-order term do not influence the degree of singularity of the solution. Therefore, 
it suffices to study the homogeneous principal transmission problem with a right-hand side $f\in\Ltwo[\Omega_L]$,
\begin{align} \label{eq:trans}
-\nabla\cdot(\bbA\nabla w) = f \;\;\;
    \hbox{in}\;\;\Omega_L, \quad
w =0 \;\;\; \hbox{on}\;\;\partial\Omega_L. 
\end{align}
The regularity of $w$ is determined by eigenvalues of local Mellin pencils near vertices of the partition $\Cp_L$ (cf. \cite{Nicaise1994a}). Near a vertex $\Bp\in\Cv_L$, the singular part of $w$ has the form
\begin{align} \label{eq:ws-mellin}
w_\Bp(r,\theta) = r^\lambda \phi(\lambda;\theta), 
\end{align}
where \(r=|\Bx-\Bp|>0\) and $\theta$ are the radial and angular variables in local coordinates. Here 
\[
        r^\lambda:=\exp(\lambda\ln r),\qquad \lambda\in\bbC .
\]
The admissible values of \(\lambda\) are precisely the eigenvalues of the local
Mellin pencil at \(\Bp\).



\begin{lemma}\label{lem:mellin}
Suppose $\Bp\in\Cv_L$ and $\lambda$ is an eigenvalue of the local Mellin pencil of \eqref{eq:trans} at $\Bp$. Then $\Re\lambda\notin (0,1)$. Actually, it admits
\begin{itemize} [leftmargin=5mm]
\item $(e^{2\pi\Vi\lambda}-1)(e^{-2\pi\Vi\lambda}-1)=0$ if $\Bp$ is an interior crossing point of two PML interfaces, 

\item $e^{2\Vi\lambda \pi}=1$ if $\Bp$ is an interface-boundary junction, and

\item $e^{\Vi\lambda \pi}=1$ if $\Bp$ is a corner of $B_L$.
\end{itemize}
The same statement holds with \(\bbA\) replaced by \(\bbA^*\).
\end{lemma}
\begin{proof}
We prove the assertions for \(\bbA\); the statement for \(\bbA^*\) is obtained by conjugating all stretching parameters. It is easy to verify that $\Re\lambda\notin (0,1)$, if $\lambda$ satisfies any of the three equalities. It is left to prove the three equalities for the corresponding types of $\Bp$. We refer to \cite{Nicaise1994a} for the Nicaise-S\"andig regularity theory for elliptic equations with discontinuous coefficients. Here we present the proof to identify local pencils for UPML coefficients. 



\begin{figure}[htp!]
    \centering
    \includegraphics[width=0.25\linewidth]{figs/4squares.png}\qquad
    \includegraphics[width=0.25\linewidth]{figs/2squares.png}\qquad
    \includegraphics[width=0.195\linewidth]{figs/1square.png}
    \caption{Left: interface-crossing point. Middle: interface-boundary junction. Right: a corner of $B_L$.}
    \label{fig:PL-vert}
\end{figure}

We consider nontrivial solutions to the homogeneous equation
\begin{align}\label{eq:UinQ}
\nabla\cdot(\bbA\nabla U)=0 \quad \hbox{in}\;\; 
\Omega_{\Bp} := \bigcup\left\{\ol{Q}: Q\in\Cp_L,\; \Bp\in\partial Q\right\}.
\end{align}
If $\Bp$ is an interior crossing point of two PML interfaces, there are four sectors sharing the origin, denoted by $Q_1,\cdots,Q_4$, respectively (Fig.~\ref{fig:PL-vert}: left). By coordinate translation and rotation, we can assume that the origin of local coordinate frame is at $\Bp$ and the two interfaces separating the sectors are \(x_1=0\) and \(x_2=0\), respectively.
Inside a fixed sector $Q_j$, $\bbA$ is constant and has the form
\[
\bbA= \operatorname{diag}\left(\alpha_2/\alpha_1,\,
\alpha_1/\alpha_2\right),\quad 
\alpha_1,\alpha_2\in\{1,1+i\sigma_0\}.
\]
We define $\xi_1=\alpha_1 x_1$, $\xi_2=\alpha_2x_2$, and
$\widehat U(\xi_1,\xi_2)=U(x_1,x_2)$ for \(\Bx\in Q_j\).
By the chain rule and \eqref{eq:UinQ}, we easily find that, when the solution is restricted to $Q_j$, 
\[
\Delta_{\xibf}\widehat U=0.
\]
Using separation of variables, the general form of the solution is obtained
\[
\wh U(\xibf) = C_j^+(\xi_1+\Vi\xi_2)^\lambda
+ C_j^-(\xi_1-\Vi\xi_2)^\lambda \quad 
\hbox{for all}\; C^\pm_j,\lambda\in\bbC.
\]
Therefore, restricted to $Q_j$, the solution $U$ is given by
\begin{align}\label{eq:sector-homogeneous-modes}
U(\Bx) = C_j^+(\alpha_1 x_1 +\Vi \alpha_2 x_2)^\lambda
+C_j^-(\alpha_1 x_1-\Vi \alpha_2 x_2)^\lambda
\quad \forall\,\Bx\in Q_j.
\end{align}
For two sectors \(Q_1, Q_2\) separated by the \(x_1\)-axis, \(\alpha_2\) is continuous across the interface, while \(\alpha_1\) is not. Denote the common value of \(\alpha_2\) by
\(\beta\), and write $\delta^\pm=C_2^\pm-C_1^\pm$.
The continuity of \(U\) across $\{x_1=0\}$ shows that 
\[
\delta^+(\Vi\beta x_2)^\lambda +\delta^-(-\Vi\beta x_2)^\lambda =0\quad
\hbox{for either $0<|x_2|< l_2$ or $l_2<|x_2|<L_2$}.
\]
Moreover, the continuity of the normal flux $(\bbA\nabla U)\cdot\Bn
=\frac{\alpha_2}{\alpha_1}\frac{\partial U}{\partial x_1}$ across \(\{x_1=0\}\) shows
\[
\delta^+(\Vi\beta x_2)^{\lambda} - \delta^-(-\Vi\beta x_2)^{\lambda} = 0.
\]
This implies
$\delta^+=\delta^-=0$, that is, $C_2^\pm=C_1^\pm$.
The same argument applies to two sectors separated by the \(x_2\)-axis.
Therefore, the expressions of the solution in the four sectors share the same coefficients, denoted by \(C^+\) and \(C^-\). The analyses also apply to the case when $\Bp$ is either an interface-boundary junction or a corner of $B_L$. 



Now we prove the first equality of the lemma for $\Bp$ being an interface-crossing point.
By rotating the local coordinate frame, we can assume that $Q_1 = B_l$ and is contained in the first quadrant (see Fig.~\ref{fig:PL-vert}: left). Using polar coordinates $x_1=r\cos\theta$ and $x_2=r\sin\theta$, we can write \eqref{eq:sector-homogeneous-modes} as
\begin{align}\label{eq:Uj}
U(\Bx) =\,& r^\lambda\big[C^+(\cos\theta +\Vi \sin\theta)^\lambda +C^-(\cos\theta -\Vi \sin\theta)^\lambda\big] \notag \\ 
=\,& r^\lambda\big[C^+ e^{\Vi \lambda\theta} +C^- e^{-\Vi \lambda\theta}\big] \quad \forall\,\Bx\in \Omega_l\subset Q_1. 
\end{align}
Note that $\alpha_1=\alpha_2=1$ in $\Omega_l$. Since $U$ is periodic in $\theta$ and smooth inside $\Omega_l$, we have
\[
U|_{\theta = 2\pi+\pi/4} = U|_{\theta =\pi/4},\quad 
\left.\frac{\partial U}{\partial\theta}
\right|_{\theta = 2\pi+\pi/4}
= \left.\frac{\partial U}{\partial\theta}
\right|_{\theta =\pi/4}.
\]
Write $\wh{C}^\pm:= e^{\pm\Vi\lambda\pi/4}C^\pm$. By \eqref{eq:Uj}, the above two conditions are equivalent to
\begin{align*}
\begin{pmatrix}
e^{2\pi\Vi\lambda}-1  &  e^{-2\pi\Vi\lambda}-1 \\
e^{2\pi\Vi\lambda}-1  &  1-e^{-2\pi\Vi\lambda}
\end{pmatrix}
\binom{\wh{C}^+}{\wh{C}^-}=0 .
\end{align*}
Nonzero solutions of the system require that the determinant of the matrix vanishes, that is,
\[
(e^{2\pi\Vi\lambda}-1)(e^{-2\pi\Vi\lambda}-1) =0.
\]


Now we prove the equality for an interface-boundary junction. In this case, $\Bp$ is shared by two sectors $Q_1$ and $Q_2$ which are contained in $B_L\backslash B_l$. Again we use the local coordinate frame with $\Bp$ being the origin and $Q_1, Q_2$ in the first and second quadrants, respectively  (Fig.~\ref{fig:PL-vert}: middle). Then  $\alpha_2=1+\Vi\sigma_0$.  Without loss of generality, we can assume $\alpha_1=1+\Vi\sigma_0$ in $Q_1$ and $\alpha_1=1$ in $Q_2$. Similar to \eqref{eq:Uj}, the solution can be written as
\begin{align*}
U(\Bx) = 
\begin{cases}
r^\lambda(1+\Vi\sigma_0)^\lambda  
(C^+e^{\Vi\lambda\theta}
+C^-e^{-\Vi\lambda\theta}) &\hbox{if}\; \Bx\in Q_1, \\
C^+ r_+^\lambda e^{\Vi\lambda\theta_+}
+C^- r_-^\lambda e^{-\Vi\lambda\theta_-} & \hbox{if} \; \Bx\in Q_2,
\end{cases}
\end{align*} 
where $\Bx = r(\cos\theta,\sin\theta)$ are expressed in polar coordinates and
\[
r_\pm := \sqrt{(x_1\mp\sigma_0 x_2)^2 + x_2^2}, \quad 
\theta_\pm := \pi - \arcsin(x_2/r_\pm).
\]
It is easy to see that $\theta(\Bx) =0$ for $\Bx\in\partial Q_1\cap\{x_2=0\}$ and 
\[
r_\pm(\Bx) = r, \quad 
\theta_\pm(\Bx) =\pi \quad \forall\,
    \Bx\in\partial Q_2\cap\{x_2=0\}.
\]
The homogeneous boundary condition of $U$ on $(\partial Q_1\cup\partial Q_2)\cap \{x_2=0\}$ implies
\begin{align*}
\begin{pmatrix}
1  &  1 \\
e^{\Vi\lambda\pi}  &  e^{-\Vi\lambda\pi}
\end{pmatrix}
\binom{C^+}{C^-}=0 .
\end{align*}
Again, the vanishing determinant of the coefficient matrix yields $e^{2\Vi\lambda\pi} =1$.


Finally, if $\Bp$ is a corner of $B_L$, it is owned only by one sector $Q$ (Fig.~\ref{fig:PL-vert}: right). Using \eqref{eq:UinQ}, we have $U(\Bx)= r^\lambda (C^+e^{\Vi\lambda\theta} +C^- e^{-\Vi\lambda\theta})$ with $0< \theta< \pi/2$. The homogeneous boundary condition of $U$ on the two edges connecting $\Bp$ shows
\[
C^+ +C^-=0,\quad
C^+e^{\Vi\lambda\pi/2} +C^- e^{-\Vi\lambda\pi/2} =0.
\]
The vanishing determinant of the coefficient matrix yields $e^{\Vi\lambda\pi} =1$. The proof is finished.
\end{proof}



\begin{theorem} \label{thm:regularity-w}
Suppose $w$ is the solution to problem \eqref{eq:trans}. 
For any \(0<s<1\), there exists a solution $C(s)$ which depends only on $s$ and $\Omega_L$ such that
\begin{equation}\label{app:eq:H1s-shift}
\|w\|_{1+s,\Cp_L^{\rm obs}}\le C(s)\|f\|_{L^2(\Omega_L)}.
\end{equation} 
\end{theorem}
\begin{proof}
Since \(\Gamma\) is \(C^2\)-smooth by the assumption in \eqref{model}, it is a smooth
Dirichlet boundary component and produces no Mellin singularities. The only conical points are vertices in \(\Cv_L\). 

Define $p= 2/(2-s)$. By Lemma~\ref{lem:mellin}, the local Mellin pencil at any $\Bp\in\Cv_L$ has no eigenvalues satisfying $\Re\lambda = 2-2/p=s$. Therefore, by \cite[Theorem~4.2]{Nicaise1994a}, the solution $w$ of \eqref{eq:trans} is regular inside each $Q\in\Cp_L^{\rm obs}$, and there exists a constant $C(s)$ depending only on $Q$ and $s$ such that
\[
\N{w}_{2,p,Q} \le C(s) \N{f}_{L^p(\Omega_L)}
\le C(s) \NLtwo[\Omega_L]{f}.
\]
The proof is finished by the Sobolev embedding $W^{2,p}(Q)\hookrightarrow H^{1+s}(Q)$ in two dimensions.
\end{proof}






==> stab-source-tmp.tex <==

\section{Wavenumber-explicit stability for the truncated source problem}
\label{sec:source}

The purpose of this section is to establish wavenumber-explicit stability of UPML for the pure source problem where $D=\emptyset$ and $\supp(f)\subset B_l$. The weak formulation \eqref{eq:weak-hu} is to find $\hat{u}\in H_0^1(B_L)$ such that 
\begin{align}\label{pml-source}
\mathscr{A}_{B_L}(\hat{u},v) = (f,\Bar{v})_{B_l}
\quad \forall\,v\in\zbHone[B_L].    
\end{align}


\begingroup
\color{blue}

\subsection{Dyadic Green-kernel estimates in the mixed and PML regions}
\label{subsec:dyadic-green-estimates}

In this subsection we refine the estimates for the mixed and PML--PML parts of the Green operator.  The key observation is that the logarithmic loss in the previous estimates is not caused by the PML damping itself.  Rather, it arises from applying global absolute-value bounds to the two-dimensional Green kernel before separating the distance scales.  We avoid this loss by decomposing the kernel dyadically with respect to the real distance \(|\Bx-\By|\) and by keeping the PML-normal variable as a one-dimensional damping operator.

Let
\[
    1=\chi_{\rm low}(\Bx,\By)+\sum_{R\in\mathcal R_k}\psi_R(\Bx,\By)
      +\chi_{\rm far}(\Bx,\By)
\]
be a smooth dyadic partition such that
\[
    \operatorname{supp}\chi_{\rm low}\subset\{|\Bx-\By|\le C/k\},
    \qquad
    \operatorname{supp}\psi_R\subset\{|\Bx-\By|\simeq R\},
\]
and
\[
    \operatorname{supp}\chi_{\rm far}\subset\{|\Bx-\By|\ge R_0/2\}.
\]
Here
\[
    \mathcal R_k=\{2^m/k:\ C_0\le kR\le CkR_0\},
\]
and the cutoffs have uniformly finite overlap.  On a fixed middle-frequency
shell \(|\Bx-\By|\simeq R\), the two-dimensional Hankel asymptotic gives
\[
    |H_0^{(1)}(k\rho(\Bx,\By))|
    \le C(kR)^{-1/2}e^{-k\operatorname{Im}\rho(\Bx,\By)}.
\]
Thus the two-dimensional analogue of the denominator is the factor
\[
    (kR)^{-1/2},
\]
rather than the three-dimensional factor \(R^{-1}\).

We shall use the following elementary one-dimensional damping estimates.

\begin{lemma}[Normal damping operators]
\label{lem:normal-damping-operators}
Let \(\gamma>0\).  Define, for \(a\ge0\),
\[
    (H_\gamma f)(a)
    =
    \int_0^\infty e^{-c\gamma a(a+b)}f(b)\,db,
\]
\[
    (K_\gamma f)(a)
    =
    \int_0^\infty e^{-c\gamma(a-b)^2}f(b)\,db,
\]
and, for a fixed \(L>0\),
\[
    (O_\gamma f)(a)
    =
    \int_0^\infty e^{-c\gamma L(a+b)}f(b)\,db.
\]
Then
\[
    \|H_\gamma\|_{L^2(0,\infty)\to L^2(0,\infty)}
    +
    \|K_\gamma\|_{L^2(0,\infty)\to L^2(0,\infty)}
    \le C\gamma^{-1/2},
\]
and
\[
    \|O_\gamma\|_{L^2(0,\infty)\to L^2(0,\infty)}
    \le C\gamma^{-1}.
\]
The constants are independent of \(\gamma\).
\end{lemma}

\begin{proof}
We first estimate \(H_\gamma\).  Introduce the unitary scaling
\[
    (U_\gamma f)(x)=\gamma^{-1/4}f(x/\sqrt{\gamma})
    \quad\text{on } L^2(0,\infty).
\]
A direct change of variables gives
\[
    U_\gamma H_\gamma U_\gamma^{-1}
    =
    \gamma^{-1/2}M,
\]
where
\[
    (MF)(x)=\int_0^\infty e^{-cx(x+y)}F(y)\,dy.
\]
Since
\[
    e^{-cx(x+y)}=e^{-cx^2}e^{-cxy}
\]
and \(e^{-cx^2}\le1\), it is enough to estimate
\[
    (L_cF)(x)=\int_0^\infty e^{-cxy}F(y)\,dy.
\]
We compute
\[
    (L_c^*L_cF)(y)
    =
    \int_0^\infty e^{-cxy}
    \left(
        \int_0^\infty e^{-cxz}F(z)\,dz
    \right)dx.
\]
Changing the order of integration yields
\[
    (L_c^*L_cF)(y)
    =
    \int_0^\infty
    \left(
        \int_0^\infty e^{-cx(y+z)}\,dx
    \right)
    F(z)\,dz
    =
    \frac1c\int_0^\infty \frac{F(z)}{y+z}\,dz.
\]
Thus \(L_c^*L_c=c^{-1}\mathcal C\), where
\[
    (\mathcal CF)(y)=\int_0^\infty \frac{F(z)}{y+z}\,dz
\]
is the Carleman operator.  We use the weighted Schur test with
\[
    w(y)=y^{-1/2}.
\]
Indeed,
\[
    \int_0^\infty \frac{w(z)}{y+z}\,dz
    =
    \int_0^\infty \frac{z^{-1/2}}{y+z}\,dz.
\]
With \(z=yt\), this becomes
\[
    y^{-1/2}\int_0^\infty \frac{t^{-1/2}}{1+t}\,dt
    =
    \pi y^{-1/2}
    =
    \pi w(y).
\]
By symmetry the second Schur condition is the same.  Hence
\[
    \|\mathcal C\|_{2\to2}\le \pi,
\]
and therefore
\[
    \|L_c\|_{2\to2}\le C.
\]
Consequently
\[
    \|H_\gamma\|_{2\to2}\le C\gamma^{-1/2}.
\]

Next, \(K_\gamma\) is a Gaussian convolution operator on the half-line.  Extend
\(f\) by zero to the whole real line.  Then
\[
    |K_\gamma f(a)|
    \le
    \int_{\mathbb R} e^{-c\gamma(a-b)^2}|\tilde f(b)|\,db.
\]
Young's inequality gives
\[
    \|K_\gamma f\|_{L^2(0,\infty)}
    \le
    \|e^{-c\gamma t^2}\|_{L^1(\mathbb R)}
    \|\tilde f\|_{L^2(\mathbb R)}
    \le
    C\gamma^{-1/2}\|f\|_{L^2(0,\infty)}.
\]
Finally, \(O_\gamma\) is rank one:
\[
    (O_\gamma f)(a)
    =
    e^{-c\gamma La}
    \int_0^\infty e^{-c\gamma Lb}f(b)\,db.
\]
Therefore
\[
    \|O_\gamma\|_{2\to2}
    =
    \|e^{-c\gamma Lt}\|_{L^2(0,\infty)}^2
    \le C\gamma^{-1}.
\]
The proof is complete.
\end{proof}

We now apply these estimates to the mixed part of the Green operator.

\begin{proposition}[One-inside-one-outside dyadic estimate]
\label{prop:one-inside-one-outside-dyadic}
Let \(T_R^{\rm mix}\) be the part of the Green operator whose kernel is
localized by \(\psi_R(\Bx,\By)\), and in which one of \(x,y\) belongs to \(B_l\)
and the other belongs to \(B_l^c\).  Then, for every middle-frequency shell,
\[
    \|T_R^{\rm mix}\|_{L^2\to L^2}
    \le C\frac{R}{k}.
\]
\end{proposition}

\begin{proof}
It is enough to consider the case \(x\in B_l^c\), \(y\in B_l\), since the
opposite case is the adjoint estimate.  We decompose \(B_l^c\) into side cells
and corner cells.

First suppose \(x\) lies in the right side cell
\[
    S_1^+=\{x_1>l_1,\ |x_2|<l_2\},
    \qquad y\in B_l.
\]
Write
\[
    x_1=l_1+a,\qquad y_1=l_1-b,
    \qquad a\ge0,\quad b\ge0.
\]
The variable \(b\) is actually bounded, but we extend functions by zero to the
half-line.  In the first coordinate,
\[
    \delta_1=x_1-y_1=a+b,
\]
and
\[
    S_1=\int_{y_1}^{x_1}\sigma_1(t)\,dt=\sigma_0a.
\]
Hence
\[
    \delta_1S_1=\sigma_0a(a+b).
\]
Using
\[
    \operatorname{Im}\rho(\Bx,\By)
    \ge
    c\frac{\delta_1S_1+\delta_2S_2}{|\Bx-\By|}
\]
and \(|\Bx-\By|\simeq R\), we get
\[
    e^{-k\operatorname{Im}\rho(\Bx,\By)}
    \le
    e^{-c(k/R)a(a+b)}.
\]
Thus, on the shell,
\[
    |K_R(\Bx,\By)|
    \le
    C(kR)^{-1/2}
    e^{-c(k/R)a(a+b)}
    \mathbf 1_{\{|\Bx-\By|\simeq R\}}.
\]
Let \(u=x_2\) and \(v=y_2\).  For an upper bound we use
\[
    \mathbf 1_{\{|\Bx-\By|\simeq R\}}
    \le
    \mathbf 1_{\{|u-v|\le CR\}}.
\]
For fixed \(a,b\), the tangential operator is bounded on \(L^2\) by Young's
inequality:
\[
    (kR)^{-1/2}\|\mathbf 1_{\{|t|\le CR\}}\|_{L^1(\mathbb R)}
    \le
    C(kR)^{-1/2}R
    =
    C\left(\frac{R}{k}\right)^{1/2}.
\]
The remaining normal operator is \(H_\gamma\) with
\[
    \gamma=\frac{k}{R}.
\]
By Lemma~\ref{lem:normal-damping-operators},
\[
    \|H_{k/R}\|_{2\to2}
    \le
    C\left(\frac{R}{k}\right)^{1/2}.
\]
Multiplying the tangential and normal bounds gives
\[
    \|T_R^{S_1^+\times B_l}\|_{2\to2}
    \le
    C\left(\frac{R}{k}\right)^{1/2}
     \left(\frac{R}{k}\right)^{1/2}
    =
    C\frac{R}{k}.
\]
The other side cells are identical up to reflection and permutation of
coordinates.

Now suppose \(x\) lies in a corner cell, for instance
\[
    C^{++}=\{x_1>l_1,\ x_2>l_2\},
    \qquad y\in B_l.
\]
Write
\[
    x_j=l_j+a_j,\qquad y_j=l_j-b_j,
    \qquad a_j,b_j\ge0,\quad j=1,2.
\]
Both coordinates are crossing coordinates, and therefore
\[
    \operatorname{Im}\rho(\Bx,\By)
    \ge
    c\frac{
        a_1(a_1+b_1)+a_2(a_2+b_2)
    }{R}.
\]
The two normal crossing operators each contribute
\[
    \left(\frac{R}{k}\right)^{1/2}.
\]
Their product is \(R/k\).  The Hankel factor \((kR)^{-1/2}\) is bounded on the
middle-frequency range \(kR\ge C_0\), and hence it can only improve the
estimate.  Thus every corner--physical pair also satisfies
\[
    \|T_R\|_{2\to2}\le C\frac{R}{k}.
\]
Since the number of side and corner cells is finite, the proposition follows.
\end{proof}

Next we estimate the part where both points lie in the PML region.

\begin{proposition}[PML--PML dyadic estimate]
\label{prop:pml-pml-dyadic}
Let \(T_R^{\rm pml}\) be the part of the Green operator whose kernel is
localized by \(\psi_R(\Bx,\By)\), and in which both \(x,y\) lie in \(B_l^c\).
Then
\[
    \|T_R^{\rm pml}\|_{L^2\to L^2}
    \le C\frac{R}{k}.
\]
\end{proposition}

\begin{proof}
We decompose \(B_l^c\) into the four side cells and the four corner cells.  The
only critical PML--PML self-pair is a side cell paired with itself.  For
example, let
\[
    x,y\in S_1^+
    =
    \{x_1>l_1,\ |x_2|<l_2\}.
\]
Write
\[
    x_1=l_1+a,\qquad y_1=l_1+b,
    \qquad a,b\ge0.
\]
Then
\[
    \delta_1=x_1-y_1=a-b,
    \qquad
    S_1=\sigma_0(a-b),
\]
and hence
\[
    \delta_1S_1=\sigma_0(a-b)^2.
\]
On the shell \(|\Bx-\By|\simeq R\),
\[
    e^{-k\operatorname{Im}\rho(\Bx,\By)}
    \le
    e^{-c(k/R)(a-b)^2}.
\]
Let \(u=x_2\) and \(v=y_2\).  As in the mixed case,
\[
    |K_R(\Bx,\By)|
    \le
    C(kR)^{-1/2}
    e^{-c(k/R)(a-b)^2}
    \mathbf 1_{\{|u-v|\le CR\}}.
\]
For fixed \(a,b\), the tangential Young estimate gives
\[
    C(kR)^{-1/2}R
    =
    C\left(\frac{R}{k}\right)^{1/2}.
\]
The normal same-side Gaussian operator is \(K_\gamma\), with
\[
    \gamma=\frac{k}{R}.
\]
By Lemma~\ref{lem:normal-damping-operators},
\[
    \|K_{k/R}\|_{2\to2}
    \le
    C\left(\frac{R}{k}\right)^{1/2}.
\]
Thus
\[
    \|T_R^{S_1^+\times S_1^+}\|_{2\to2}
    \le
    C\frac{R}{k}.
\]

All remaining PML--PML pairs are easier.  If the pair has two crossing or
same-side coordinates, then the two normal estimates give
\[
    \left(\frac{R}{k}\right)^{1/2}
    \left(\frac{R}{k}\right)^{1/2}
    =
    \frac{R}{k}.
\]
If the pair contains an opposite-side coordinate, then the operator \(O_{k/R}\)
already gives \(R/k\).  The remaining coordinate contributes at most a bounded
factor by Young's inequality and the middle-frequency bound on the Hankel
factor.  Since there are only finitely many hard-cell pairs, the desired
estimate follows.
\end{proof}

Combining the two dyadic estimates gives the logarithm-free bound for the
mixed and PML parts.

\begin{corollary}[No-logarithm estimate for \(I_2\) and \(I_3\)]
\label{cor:no-log-I2-I3}
Let \(I_2\) denote the one-inside-one-outside part and \(I_3\) the PML--PML
part in the decomposition of the Green potential.  Then
\[
    |I_2|+|I_3|
    \le
    Ck^{-1}
    \|F_1\|_{L^2(\mathbb R^2)}
    \|v\|_{L^2(\mathbb R^2)}.
\]
\end{corollary}

\begin{proof}
For each middle-frequency shell, Propositions
\ref{prop:one-inside-one-outside-dyadic} and
\ref{prop:pml-pml-dyadic} give the bound \(CR/k\).  Hence
\[
    \sum_{R\in\mathcal R_k}\frac{R}{k}
    =
    \frac1k\sum_{R\in\mathcal R_k}R
    \le
    \frac{C}{k},
\]
because the dyadic shells cover only a fixed bounded distance range.  The low
frequency and far-field parts are controlled by the preceding local and
far-field estimates.  Therefore no factor \(\log k\) appears.
\end{proof}

\begin{remark}[Why the logarithm disappears]
The old estimate treats the two-dimensional Green kernel too globally and
therefore effectively sums one constant over all dyadic shells.  This produces
\(\sum_R1\simeq \log k\).  The dyadic argument above gives, on each shell,
\[
    \frac{R}{k},
\]
not \(1/k\).  Hence the final summation is
\[
    \sum_R \frac{R}{k}
    =
    \frac1k\sum_R R
    \le
    \frac{C}{k}.
\]
The critical two-dimensional mechanism is
\[
    \underbrace{(kR)^{-1/2}}_{\text{Hankel half-power}}
    \underbrace{R}_{\text{tangential Young}}
    \underbrace{(R/k)^{1/2}}_{\text{normal damping}}
    =
    \frac{R}{k}.
\]
This is specific to the two-dimensional Hankel kernel.  It should not be
identified with the three-dimensional factor \(1/\rho\).
\end{remark}

\endgroup



\subsection{Useful estimates for $G(\tilde\Bx,\tilde\By)$}

Fist we prove some useful estimates concerning $G(\tilde\Bx,\tilde\By)$. 
The technique is to estimate $\wt G(\Bx,\By)$ for two cases: $\Bx,\By\in B_l^c$, and one in $B_l$ and the other in $B_l^c$, separately.
The first case is obtained by estimates for free-space Helmholtz equation, while the other relies on both near-field estimates and exponential decay of the stretched Green's function. 
\vspace{1mm}

\begin{lemma}\label{lem:far-field}
Let $R$ be defined in Lemma~\ref{lem:Imrho-large-sep}. There exists a constant $C>0$ which depend on $R$ and $\sigma_0$, but not on $k$, such that, for $j=0,1,2$,
\begin{align}
&\sup_{\Bx\in\bbR^2}\int_{\{\By\in\bbR^2:\ |\Bx-\By|\ge R\}}
\big|\nabla^j_{\Bx}G(\tilde\Bx,\tilde\By)\big|\,{\D} \By
\le Ck^{j-2}\big(1+\sqrt{kR}\big) e^{-\frac{1}{8}\sigma_0kR}, 
    \label{eq:G-tail-L1}\\    
&\int_{\Bx\in B_l}\int_{\{\By\in\bbR^2:\ |\Bx-\By|\ge R\}}
\big|\nabla_{\Bx}^j G(\tilde\Bx,\tilde\By)\big|^2\,{\D} \By\,{\D} \Bx
\le	Ck^{j-2}e^{-\frac{1}{4}\sigma_0kR}.  \label{eq:G-tail-L2}
\end{align}
\end{lemma}
\begin{proof}
The proof is based on the results in Lemma~\ref{lem:decay-stretchedG}. We only prove the lemma for $j=0$. The proofs for $j=1$ and $2$ are parallel.

For $|\Bx-\By|> R$, from Lemmas~\ref{lem:decay-stretchedG} and \ref{lem:Imrho-large-sep}, we know that
\begin{equation}\label{eq:G-farfield-exp}
\big|G(\tilde\Bx,\tilde\By)\big| \le C(k|\Bx-\By|)^{-1/2}
e^{-\tfrac18 k\sigma_0\,|\Bx-\By|}.
\end{equation}
Using the polar coordinates centered at $\Bx$, we obtain
\begin{align*}
\int_{|\Bx-\By|\ge R}\big|G(\tilde\Bx,\tilde\By)\big|\,{\D} \By
\le C\int_R^\infty (kr)^{-1/2}e^{-\frac{1}{8}\sigma_0 kr} r{\D} r 
=Ck^{-2}\int_{kR}^\infty e^{-\frac{1}{8}\sigma_0t} t^{1/2}{\D} t.
\end{align*}
Write $t=kR+s$ with $s\ge0$. Then
\[
\int_{kR}^\infty e^{-\frac{1}{8}\sigma_0t} t^{1/2}{\D} t
\le e^{-\frac{1}{8}\sigma_0kR} \int_0^\infty e^{-\frac{1}{8}\sigma_0 s}
\big(\sqrt{s}+\sqrt{kR}\big){\D} s
\le C \big(1+\sqrt{kR}\big) e^{-\frac{1}{8}\sigma_0kR}.
\]
This yields \eqref{eq:G-tail-L1}.


Similarly, we use \eqref{eq:G-farfield-exp} and find that
\begin{align*}
\int_{|\Bx-\By|\ge R}\big|G(\tilde\Bx,\tilde\By)\big|^2{\D} \By
\le Ck^{-1}\int_R^\infty e^{-\frac{1}{4}\sigma_0 kr}{\D} r 
\le Ck^{-2}e^{-\frac{1}{4}\sigma_0kR}.
\end{align*}
Since $B_l$ is bounded independent of $k$, \eqref{eq:G-farfield-exp} is a direct consequence of the above inequality.
\end{proof}

\begin{lemma}\label{lem:nearfield-L2}
Define $D_1 :=\{(\Bx,\By)\in B_l^c\times B_l:|\Bx-\By|\le R\}$ and $D_2 :=\{(\Bx,\By):(\By,\Bx)\in D_1\}$. There exists a constant $C>0$ independent of $k$ such that, for $j=0,1,2$, 
\begin{equation}\label{eq:nearfield-L2}
\big\|\wt G\big\|_{H^j(D_1)}
+\big\|\wt G\big\|_{H^j(D_2)}\le C k^{j-1}\ln k.
\end{equation} 
\end{lemma}
\begin{proof}
Again, we only prove the lemma for $j=0$ by using Lemma~\ref{lem:decay-stretchedG}. The proofs for $j=1$ and $2$ are parallel.


We first estimate $\wt G(\Bx,\By)=G(\tilde\Bx,\By)$ for $(\Bx,\By)\in D_1$. Define $r(\Bx) = \max\limits_{j=1,2}\, (|x_j|-l_j)$ and
\[
\big(\xi(\Bx,\By),\, \eta(\Bx,\By)\big) = 
\begin{cases}
\big(|x_1-y_1|,\, l_1-\Sign(x_1)y_1 \big)  & \hbox{if}\;\; |x_1|-l_1 \ge |x_2|-l_2, \\
\big(|x_2-y_2|,\, l_2-\Sign(x_2)y_2\big) & \hbox{otherwise.}
\end{cases}
\]
For convenience, we use the abbreviations $\xi=\xi(\Bx,\By)$, $\eta=\eta(\Bx,\By)$, $r=r(\Bx)$, and $d = \sqrt{r\xi}$. 
By the complex transformation \eqref{eq:stretch}--\eqref{eq:sigma-assump}, it is easy to verify that 
\begin{align}\label{xi-r-eta}
\xi =r + \eta \le |\Bx-\By|,\quad 
\sigma_0d^2 = (x_j-y_j)\int_{y_j}^{x_j}\sigma_j(t)\D t \;\;
\hbox{for}\; j=1\; \hbox{or}\; 2.
\end{align}
Moreover, we define $A:=\tfrac12 \sigma_0kd^2$ and $g(s):=s e^{-As^2}$. From \eqref{eq:Imrho-lower} and \eqref{eq:G-decay}, we have 
\begin{align}\label{max-g}
|G(\tilde{\Bx},\By)|\le C k^{-1/2}|\Bx-\By|^{-1/2}
e^{-A|\Bx-\By|^{-1}} \le Ck^{-1/2} \max_{0\le s\le \xi^{-1/2}} g(s).
\end{align}
The function $g(s)$
attains its maximal value $(2A)^{-1/2} e^{-1/2}$ at $s_0 =(2A)^{-1/2}=(\sigma_0k)^{-1/2}d^{-1}$. 
 

If $r < (\sigma_0 k)^{-1}$, then $s_0>\xi^{-1/2}$. The constrained maximum on the right-hand side of \eqref{max-g} is attained at the endpoint $s = \xi^{-1/2}$. Therefore, 
\begin{align}\label{d-small}
|G(\tilde{\Bx},\By)|\le C k^{-1/2}\xi^{-1/2}
e^{-\frac{1}{2}\sigma_0 k \xi} 
\le C k^{-1/2}\xi^{-1/2} \quad
\hbox{if}\;\; r < (\sigma_0 k)^{-1}.
\end{align}
Otherwise, the maximum is attained at $s_0\le \xi^{-1/2}$. This shows
\begin{align}\label{d-large}
|G(\tilde{\Bx},\By)|\le C k^{-1/2} (2A)^{-1/2} 
\le C k^{-1}r^{-1/2}\xi^{-1/2}\quad
\hbox{if}\;\; r \ge (\sigma_0 k)^{-1}.
\end{align}

Write $l = \max\{l_1,l_2\}$. 
By \eqref{xi-r-eta} and direct calculations, we find that
\begin{align*}
\int_{B_l} \frac{1}{\xi(\Bx,\By)}\D\By 
= \int_{B_l} \frac{1}{r(\Bx) + \eta(\Bx,\By)}\D\By 
\le C \int_0^{2l} \frac{1}{r(\Bx)+ t}\D t
= C\ln \bigg(1+ \frac{2l}{r(\Bx)}\bigg) \quad \forall\,\Bx\in B_l^c.
\end{align*}
We split $B_l^c$ into the union of two disjoint sub-domains
\[
B^c_{l,-}:=\big\{\Bx\in B_l^c: r(\Bx)< (\sigma_0k)^{-1}\big\}, \quad
B^c_{l,+}:=\big\{\Bx\in B_l^c: r(\Bx)\ge (\sigma_0k)^{-1}\big\}.
\]
Then the $\Ltwo[D_1]$-norm of $\wt G$ is estimated as follows
\begin{align*}
\int_{D_1} |\wt{G}(\Bx,\By)|^2\D\By\D\Bx 
\le\,&  \frac{C}{k} \int_{B_{l,-}^c} \bigg(\int_{B_l} 
\frac{1}{\xi(\Bx,\By)} \D\By\bigg)\D\Bx 
+ \frac{C}{k^2} \int_{B_{l,+}^c} \frac{1}{r(\Bx)}
\bigg(\int_{B_l} \frac{1}{\xi(\Bx,\By)} \D\By\bigg)\D\Bx \\
\le\,&  \frac{C}{k} \int_{B_{l,-}^c} \ln \bigg(1+ \frac{2l}{r(\Bx)}\bigg)\D\Bx 
+ \frac{C}{k^2} \int_{B_{l,+}^c} \frac{1}{r(\Bx)}
\ln \bigg(1+ \frac{2l}{r(\Bx)}\bigg)\D\Bx \\
\le\,&  \frac{C}{k} \int_0^{1/(\sigma_0k)} 
\ln \bigg(1+ \frac{2l}{t}\bigg)\D t 
+ \frac{C}{k^2} \int_{1/(\sigma_0k)}^R 
\frac{1}{t} \ln \bigg(1+ \frac{2l}{t}\bigg)\D\Bx \\
\le\,& C\frac{\ln k}{k^2} + C\frac{(\ln k)^2}{k^2}.
\end{align*}
This proves the estimate of $\big\|\wt G\big\|_{\Ltwo[D_1]}$ in \eqref{eq:nearfield-L2}. 

Note from \eqref{eq:A-J} that the Jacobian $J=\det(\bbA)$ is bounded independent of $k$. The estimate of $\big\|\wt G\big\|_{\Ltwo[D_2]}$ is parallel. The proof is finished.
\end{proof}
\vspace{1mm}

\begin{lemma}\label{lem:mixed-field}
Let $B_R(\Bx)$ denotes the ball whose radius and center are $R$ and $\Bx$, respectively. There exists a constant $C>0$ independent of \(k\) such that, for $j=0,1,2$,
\begin{equation}\label{eq:unified-trunc-bound} 
\sup_{\Bx \in B_l^c}\int_{B_l^c\cap B_R(\Bx)}
\big|\nabla_{\Bx}^jG(\tilde\Bx,\tilde\By)|\,{\D} \By\le Ck^{j-1}\ln k .
\end{equation}
\end{lemma}
\begin{proof} 
Again, we only prove the lemma for $j=0$ by using Lemma~\ref{lem:decay-stretchedG}. The proofs for $j=1$ and $2$ are parallel. The arguments are similar to those in the proof of Lemma~\ref{lem:nearfield-L2}. 


In the present case, both $\Bx$ and $\By$ are in $B_l^c$. 
We define $r(\Bx,\By)>0$ such that 
\begin{align} \label{eq:r}
r^2(\Bx,\By) := \max_{j=1,2}\,\zeta(x_j,y_j),\quad
\zeta(x_j,y_j): =\frac{x_j-y_j}{\sigma_0}
\int_{y_j}^{x_j}\sigma_j(t) \D t.
\end{align} 
Let $j\in \{1,2\}$ satisfy $\zeta(x_j,y_j) \ge \zeta(x_{3-j},y_{3-j})$. This implies $\max\{|x_j|,|y_j|\}>l_j$. By \eqref{eq:xjyj}, we have 
\begin{align*}
\zeta(x_j,y_j) =  |x_j-y_j| \times 
\begin{cases}
\max\{|x_j|,|y_j|\} -l_j  & \hbox{if}\;\; \min\{|x_j|,|y_j|\}<l_j, \\
|x_j-y_j|  & \hbox{if}\;\; \min\{|x_j|,|y_j|\}>l_j  
    \; \hbox{and}\; x_jy_j>0, \\
|x_j-y_j| -2l_j  & \hbox{if}\;\; \min\{|x_j|,|y_j|\} >l_j  
    \; \hbox{and}\; x_jy_j<0.
\end{cases}        
\end{align*}
It is clear that $r(\Bx,\By)\le |\Bx-\By|$.
 
 

 
Write $A = \frac{1}{2}\sigma_0 k r^2$ with $r=r(\Bx,\By)$. From \eqref{eq:Imrho-lower} and \eqref{eq:G-decay}, we have 
\[
|G(\tilde\Bx,\tilde\By)| \le C(k|\Bx-\By|)^{-1/2}
e^{-A|\Bx-\By|^{-1}}
\le Ck^{-1/2} \max_{0\le s\le r^{-1/2}} (s e^{-A s^2}).
\]
By arguments similar to \eqref{d-small} and \eqref{d-large}, we obtain
\begin{align*} 
|G(\tilde{\Bx},\tilde\By)|\le C \times
\begin{cases}
k^{-1/2}r^{-1/2} & \hbox{if}\;\; r < (\sigma_0 k)^{-1}, \\
k^{-1}r^{-1} & \hbox{otherwise.}
\end{cases}
\end{align*}
Note that the length of $\partial B_R(\Bx)=2\pi R= 8\sqrt{2} 
\pi\max\{l_1,l_2\}$ and $J=\det(\bbA)$ is bounded. There exists a generic constant $C>0$ which depends on $R$, but not on $k$, such that
\begin{align*}
\int_{B_l^c\cap B_R(\Bx)}|G(\tilde\Bx,\tilde\By)|\,{\D} \By
\le Ck^{-1/2}\bigg(\int_0^{1/(\sigma_0k)} r^{-1/2}\D r
+ k^{-1/2}\int_{1/(\sigma_0k)}^{2R} r^{-1}\D r\bigg)  
\le Ck^{-1}\ln k.
\end{align*}
The proof is finished.
\end{proof}
 

\subsection{Inf-sup condition for $\mathscr{A}_{\bbR^2}$}

Now we prove the inf-sup condition for the whole-space bilinear form $\mathscr{A}_{\bbR^2}$. Given a linear functional $F\in \Hone[\bbR^2]'$, we consider the weak problem: find $w\in\Hone[\bbR^2]$ such that
\begin{equation}\label{eq:upml-whole}
\mathscr{A}_{\bbR^2}(w,\psi) =\langle F, \psi\rangle
\quad \forall\,\psi\in H^{1}(\bbR^2).
\end{equation}

	
\begin{lemma}\label{lem:upml-whole}
Problem \eqref{eq:upml-whole} has a unique solution $w\in H^{1}(\bbR^2)$. Moreover, there exists a constant $C>0$ independent of $k$ such that
\begin{equation}\label{eq:chen-lemma3.3-stab}
\|w\|_{H^{1}(\bbR^2)}\le C k\ln k\|F\|_{H^{1}(\bbR^2)'}.
\end{equation}
\end{lemma}
\begin{proof}
It is known that \eqref{eq:upml-whole} has a unique solution under
the condition \eqref{eq:sigma-assump}  (cf. e.g.\ \cite{KimPasciak2010}). It is left to show the $k$-explicit stability.

Note that $\Re\big(\alpha_{1}(x_{1})/\alpha_{2}(x_{2})\big)\ge (1+\sigma_0^2)^{-1}$ and $\Re\big(\alpha_{2}(x_{2})/\alpha_{1}(x_{1})\big)\ge (1+\sigma_0^2)^{-1}$. By the Lax-Milgram lemma, there exists a unique solution $w_0\in H^{1}(\bbR^2)$ to the problem
\begin{equation}\label{eq:chen-3.6}
\int_{\bbR^2}(\bbA\nabla w_0\cdot\nabla\psi
+k^{2}J w_0\psi) =\langle F, \psi\rangle
\quad \forall\,\psi\in H^{1}(\bbR^2),
\end{equation}
and it admits 
\begin{align}\label{est-w0}
\|w_0\|_{H^{1}(\bbR^2)}\le C\|F\|_{H^{1}(\bbR^2)'}.    
\end{align}
Define $F_{1}:=k^{2}J^{-1}w_0+k^{2}w_0$ and introduce the Newtonian potential
\begin{equation}\label{eq:chen-3.7}
\Phi(\Bx):=\int_{\bbR^2} \wt G(\Bx,\By)F_{1}(\By)\,{\D} \By .
\end{equation}
Then equation \eqref{eq:pml-fundamental} shows that $\Phi$ satisfies
\begin{equation}\label{eq:Phi}
\mathscr{A}_{\bbR^2}(\Phi,\psi) =\int_{\bbR^2}JF_{1}\psi 
\quad \forall\,\psi\in H^{1}(\bbR^2).
\end{equation}
Clearly $w_0+\Phi$ solves \eqref{eq:upml-whole}.
The uniqueness of solution shows $w=w_0+\Phi$. 

Suppose $v\in L^{2}(\bbR^2)$ and consider the integral
\begin{align} \label{eq:Phi-v}
\int_{\bbR^2}\Phi(\Bx) v(\Bx)\D\Bx = \int_{\bbR^2} 
\int_{\bbR^2} \wt{G}(\Bx,\By) 
F_{1}(\By)v(\Bx){\D}\By{\D}\Bx 
= I_1 + I_2 +I_3,
\end{align}
where
\begin{align*}
I_1 =\,& \int_{B_l}\int_{B_l} G(\Bx,\By) 
F_{1}(\By)v(\Bx){\D}\By{\D}\Bx , \\
I_2 =\,&  \bigg(\int_{B_l^c}\int_{B_l} 
+  \int_{B_l}\int_{B_l^c}\bigg) \wt G(\Bx,\By) 
F_{1}(\By)v(\Bx){\D}\By{\D}\Bx, \\
I_3 =\,& \int_{B_l^c}\int_{B_l^c} \wt G(\Bx,\By) 
F_{1}(\By)v(\Bx){\D}\By{\D}\Bx .
\end{align*}
To estimate $I_1$, we extend $F_1|_{B_l}$ by zero to $B_l^c$ and denote the extension by $\tilde{F}_1$. Define
\[
\Phi_1 := \int_{B_l}G(\Bx,\By) F_1(\By)\D\By
= \int_{\bbR^2}G(\Bx,\By) \tilde{F}_1(\By)\D\By
\]
The Newtonian potential $\Phi_1$ solves the scattering problem in free space 
\begin{align*}
\Delta \Phi_1 + k^2 \Phi_1 = -\tilde{F}_1 \;\;  \text{in}\; \bbR^2,  \quad
r^{1/2}\big(\partial_r \Phi_1-\Vi k \Phi_1\big)\to 0
\;\;  \text{as}\; r\to\infty.
\end{align*} 
By \cite[Lemma~3.5 ]{MelenkSauter2010}, there exists a constant $C>0$ independent of $k$  such that
\begin{equation*}
k^{-1}\SN{\Phi_1}_{H^2(B_l)} +\|\Phi_1\|_{H^1(B_l)} 
\le C\big\|\tilde F_1\big\|_{L^2(\bbR^2)} = C\|F_1\|_{L^2(B_l)}.
\end{equation*}
An application of the Cauchy-Schwarz inequality yields
\begin{equation}\label{est-I1}
|I_1|\le \|\Phi_1\|_{L^2(B_l)}\|v\|_{L^2(B_l)}
\le Ck^{-1}\|F_1\|_{L^2(B_l)}\|v\|_{L^2(B_l)} .
\end{equation}

Next we estimate $I_2$. Recalling \eqref{eq:G-tail-L2} and  Lemma~\ref{lem:nearfield-L2}, we have
\begin{align*}
\int_{B_l^c}\int_{B_l}\SN{G(\tilde\Bx,\tilde\By)}^2\D\By\D\Bx 
\le\,& \int_{D_1}\SN{G(\tilde\Bx,\tilde\By)}^2\D\By\D\Bx 
+ \int_{B_l}\bigg(\int_{B_l^c\backslash B_R(\By)} \SN{G(\tilde\Bx,\tilde\By)}^2\D\Bx\bigg)\D\By \\
\le\,& C(k^{-1}\ln k)^2 + Ck^{-2}e^{-\frac{1}{4}\sigma_0kR}.
\end{align*}
Since $G(\tilde\Bx,\tilde\By) =G(\tilde\By,\tilde\Bx)$, the first term of $I_2$ can be estimated as follows 
\begin{align*} 
\bigg|\int_{B_l^c}\int_{B_l}\wt G(\Bx,\By) 
F_{1}(\By)v(\Bx){\D}\By{\D}\Bx\bigg| \le\,&
\NLtwo[B_l^c]{v} \NLtwo[B_l]{F_1} \bigg(\int_{B_l^c}\int_{B_l}|G(\tilde\Bx,\By)|^2\D\By\D\Bx \bigg)^{1/2} \\ 
\le\,& Ck^{-1}\ln k \NLtwo[B_l^c]{v} \NLtwo[B_l]{F_1} .
\end{align*}
The second term of $I_2$ can be estimated similarly. We obtain
\begin{align}\label{est-I2} 
|I_2|\le  Ck^{-1}\ln k \NLtwo[B_l^c]{v} \NLtwo[B_l]{F_1} .
\end{align}

For $I_3$, we use the Cauchy-Schwarz inequality and the identity $G(\tilde\Bx,\tilde\By) = G(\tilde\By,\tilde\Bx)$. It admits
\begin{align*}
|I_3|\le\,& \NLtwo[B_l^c]{v} \NLtwo[B_l^c]{F_1} \bigg(\int_{B_l^c}\int_{B_l^c}|\wt G(\Bx,\By)|^2\D\By\D\Bx \bigg)^{1/2} \\
\le\,& C\NLtwo[B_l^c]{v} \NLtwo[B_l^c]{F_1} \bigg[\int_{B_l^c} 
\Big(\sup_{\By\in B_l^c} |G(\tilde\Bx,\tilde\By)|\Big)
\bigg(\int_{B_l^c}|G(\tilde\Bx,\tilde\By)|\D\By\bigg)
\D\Bx \bigg]^{1/2} \\
\le\,& C\NLtwo[B_l^c]{v} \NLtwo[B_l^c]{F_1} 
\sup_{\Bx\in B_l^c} \int_{B_l^c}|G(\tilde\Bx,\tilde\By)|\D\By.
\end{align*}
The supremum can be estimate by using \eqref{eq:G-tail-L1} and Lemma~\ref{lem:mixed-field}. For any $\Bx\in B_l^c$, we have
\begin{align*}
\int_{B_l^c}|G(\tilde\Bx,\tilde\By)|\D\By
\le\,& \int_{B_l^c\cap B_R(\Bx)}|G(\tilde\Bx,\tilde\By)|\D\By
+ \int_{B_l^c\backslash B_R(\Bx)}|G(\tilde\Bx,\tilde\By)|\D\By \\
\le\,& Ck^{-1}\ln k + Ck^{-2}\big(1+\sqrt{kR}\big) e^{-\frac{1}{8}\sigma_0kR}.
\end{align*}
Therefore, we obtain
\begin{align}\label{est-I3}
|I_3| \le C k^{-1}\ln k \NLtwo[B_l^c]{v} \NLtwo[B_l^c]{F_1} .
\end{align}
Finally, inserting \eqref{est-I1}, \eqref{est-I2}, and \eqref{est-I3} into \eqref{eq:Phi-v}, we obtain
\begin{align*}
\bigg|\int_{\bbR^2}\Phi(\Bx) v(\Bx)\D\Bx\bigg| \le C k^{-1}\ln k \NLtwo[\bbR^2]{v} \NLtwo[\bbR^2]{F_1}. 
\end{align*}
This implies $\|\Phi\|_{L^2(\bbR^2)}\le C k^{-1}\ln k \|F_1\|_{L^2(\bbR^2)}$. 


Replace $\Phi$ and $\wt{G}(\Bx,\By)$ in \eqref{eq:Phi-v} with $\nabla\Phi$ and $\nabla_{\Bx}\wt{G}(\Bx,\By)$, respectively. The estimate of $\NLtwov[\bbR^2]{\nabla\Phi}$ can be derived similarly following the lines in the estimate of $\NLtwo[\bbR^2]{\Phi}$ and using the estimates of $\nabla_{\Bx}G(\tilde\Bx,\tilde\By)$ in Lemmas~\ref{lem:far-field}, \ref{lem:nearfield-L2}, and \ref{lem:mixed-field}. This yields
\begin{equation}\label{eq:gradPhi-L2}
\|\nabla\Phi\|_{L^2(\bbR^2)}\le C\ln k\|F_1\|_{L^2(\bbR^2)} .
\end{equation}
Recalling that $\|F_{1}\|_{L^{2}(\bbR^2)}\le Ck^{2}\|w_0\|_{L^{2}(\bbR^2)}\le Ck\,\|F\|_{H^{1}(\bbR^2)'}$, we have
\begin{equation*}
\|\Phi\|_{H^{1}(\bbR^2)}\le Ck\ln k\|F\|_{H^1(\bbR^2)'}.
\end{equation*}
The proof is finished by using \eqref{est-w0} and the identity $w=w_0+\Phi$.
\end{proof}
	
	
\begin{theorem}\label{thm:infsup-R2}
There exists a constant $\mu_0>0$ independent of $k$ such that
\begin{equation}\label{eq:infsup-R2}
\sup_{0\neq \psi\in H^1(\bbR^2)}
\frac{|\mathscr{A}_{\bbR^2}(\phi,\psi)|}{\|\psi\|_{H^1(\bbR^2)}}
\ge \frac{\mu_0}{k\ln k}\|\phi\|_{H^1(\bbR^2)}
\quad \forall\,\phi\in H^1(\bbR^2).
\end{equation}
\end{theorem}
\begin{proof}
It is easy to see that the bilinear form $a$ is continuous on $\Hone[\bbR^2]$. For \(\phi\in H^1(\bbR^2)\), we define a linear functional \(F\in H^{1}(\bbR^2)'\) as follows
\[
\langle F,\psi\rangle:=
\mathscr{A}_{\bbR^2}(\phi,\psi)	\quad \forall\,\psi\in H^1(\bbR^2).
\]
By Lemma~\ref{lem:upml-whole}, \(\phi\) is the unique solution to the weak problem
\[
\mathscr{A}_{\bbR^2}(\phi,\psi)=\langle F,\psi\rangle	\quad \forall\,\psi\in H^1(\bbR^2).
\]
The stability estimate in Lemma~\ref{lem:upml-whole} shows that
\begin{align*}
\|\phi\|_{H^1(\bbR^2)}\le C k\ln k\|F\|_{H^{1}(\bbR^2)'}
=C k\ln k\sup_{0\neq \psi\in H^1(\bbR^2)}
\frac{|\mathscr{A}_{\bbR^2}(\phi,\psi)|}{\|\psi\|_{H^1(\bbR^2)}}.
\end{align*}
The proof is finished by setting $\mu_0 = 1/C$.
\end{proof}
	
\subsection{Inf-sup condition for $\mathscr{A}_{B_L}$}

Next we derive the inf-sup condition for $\mathscr{A}_{B_L}$ on the truncated domain. We adopt the reflection argument in the proof of \cite[Theorem~5.5]{BramblePasciak2013} and specify the dependency of all stability constants on $k$.

\begin{theorem}	\label{thm:infsup-BL}
Assume $d:=\min\{d_1, d_2\}>1.2R$ and that $\sigma_0d$ is large enough. There exists a constant \(\mu_1>0\) independent of $k$ such that
\begin{equation}\label{eq:infsup-BL}
\sup_{0\neq v\in H_0^1(B_L)}
\frac{|\mathscr{A}_{B_L}(\phi,v)|}{\|v\|_{H^1(B_L)}}
\ge \frac{\mu_1}{k\ln k} \|\phi\|_{H^1(B_L)}	\quad \forall\,\phi\in H_0^1(B_L).
\end{equation}
\end{theorem}
\begin{proof}
Given $\phi\in H_0^1(B_L)$, we define a linear functional $F\in H^{-1}(B_L)$ by
\[
\langle F,\psi\rangle := \mathscr{A}_{B_L}(\phi,\psi)	
\quad\forall\,\psi\in H_0^1(B_L).
\]
It suffices to show $\|\phi\|_{H^1(B_L)}\le Ck\ln k\|F\|_{H^{-1}(B_L)}$ for a constant $C$ independent of $k$.
		
We extend $\phi$ from $B_L$ to a larger rectangle $\wt B_L:=(-L_1-d_1,\,L_1+d_1)\times(-L_2-d_2,\,L_2+d_2)$ by odd reflections. First we define $\phi_1$ on
$(-L_1-d_1,\,L_1+d_1)\times(-L_2,L_2)$ by
\begin{align*}
\phi_1(\Bx)=
\begin{cases}
-\phi(2L_1-x_1,x_2) & \hbox{if}\;\; \Bx\in (L_1,\,L_1+d_1)\times(-L_2,L_2),\\
\phi(x_1,x_2) & \hbox{if}\;\; \Bx\in [-L_1,L_1]\times(-L_2,L_2),\\
-\phi(-2L_1-x_1,x_2) & \hbox{if}\;\; \Bx\in (-L_1-d_1,\,-L_1)\times(-L_2,L_2).
\end{cases}
\end{align*}
Next we define $\tilde\phi\in H^1(\wt B_L)$ by odd reflection of $\phi_1$ across $x_2=\pm L_2$:
\begin{align*}
\tilde\phi(\Bx)=
\begin{cases}
-\phi_1(x_1,2L_2-x_2) & \hbox{if}\;\;\Bx\in (-L_1-d_1,\,L_1+d_1)\times (L_2,\,L_2+d_2),\\
\phi_1(x_1,x_2)	&  \hbox{if}\;\; \Bx\in (-L_1-d_1,\,L_1+d_1)\times [-L_2,L_2],\\
-\phi_1(x_1,-2L_2-x_2) & \hbox{if}\;\;  \Bx\in (-L_1-d_1,\,L_1+d_1)\times (-L_2-d_2,\,-L_2).
\end{cases}
\end{align*}
It is clear that $\tilde\phi\in\Hone[\wt B_L]$. Next define a linear functional $\tilde F\in H^{-1}(\wt B_L)$ by
\begin{align}\label{problem-tF}
\langle \tilde F,\psi\rangle :=	\mathscr{A}_{\wt B_L}(\tilde\phi,\psi) 
\quad	\forall\,\psi\in H_0^1(\wt B_L). 
\end{align}



To estimate the upper bound of $\tilde F$, we extend $\psi|_{\wt B_L\backslash B_L}$ to $B_L$ by reflections. First we define $\psi_1$ by even reflections a cross $x_2=\pm L_2$
\begin{align*}
\psi_1(\Bx)=
\begin{cases}
\psi(x_1,2L_2-x_2) & \hbox{if}\;\;\Bx\in (-L_1-d_1,\,L_1+d_1)\times(l_2,\,L_2),\\
0	&  \hbox{if}\;\; \Bx\in (-L_1-d_1,\,L_1+d_1)\times [-l_2,l_2],\\
\psi(x_1,-2L_2-x_2) & \hbox{if}\;\;  \Bx\in(-L_1-d_1,\,L_1+d_1)\times(-l_2,\,-L_2).
\end{cases}
\end{align*}
Clearly $\psi_1$ is continuous across the interfaces.
Next we define $\hat\psi$ by reflections of $\psi_1$ across $x_1=\pm L_1$
\begin{align*}
\hat\psi(\Bx)=
\begin{cases}
\psi(2L_1-x_1,x_2) -\psi_1(2L_1-x_1,x_2) 
    & \hbox{if}\;\; \Bx\in (l_1,\,L_1)\times(-L_2,L_2),\\
-\psi_1(x_1,x_2) & \hbox{if}\;\; \Bx\in [-l_1,l_1]\times(-L_2,L_2),\\
\psi(-2L_1-x_1,x_2) -\psi_1(-2L_1-x_1,x_2) 
    & \hbox{if}\;\; \Bx\in (-L_1,\,-l_1)\times(-L_2,L_2).
\end{cases}
\end{align*}
It is easy to check that $\hat\psi$ is continuous a cross the two interfaces $x_1=\pm l_1$. Therefore, $\hat\psi\in\Hone[B_L]$.
Since $\bbA$ and $J$ are constant in $\wt B_L\backslash\ol{B}_l$, the definitions of $\tilde\phi$ and $\hat\psi$ shows that
\begin{align*}
\langle \tilde F,\psi\rangle =\,& \mathscr{A}_{B_L}(\phi,\psi) 
+\int_{L_2\le |x_2|\le L_2+d_2}\int_{-L_1-d_1}^{L_1+d_1}
\big(\bbA\nabla\tilde\phi\cdot\nabla\psi 
-k^2\tilde\phi\psi\big)\D x_1\D x_2 \\
& +\int_{-L_2}^{L_2}\int_{L_1\le |x_1|\le L_1+d_1}
\big(\bbA\nabla\tilde\phi\cdot\nabla\psi 
-k^2\tilde\phi\psi\big)\D x_1\D x_2 \\
=\,& \mathscr{A}_{B_L}(\phi,\psi-\psi_1) 
+\int_{-L_2}^{L_2}\int_{L_1\le |x_1|\le L_1+d_1}
\big[\bbA\nabla\phi_1\cdot\nabla(\psi-\psi_1)
-k^2\phi_1(\psi-\psi_1)\big]\D x_1\D x_2 \\
=\,& \mathscr{A}_{B_L}(\phi,\psi-\psi_1-\hat\psi) .
\end{align*}
The definitions of $\psi_1$ and $\hat\psi$ imply $\psi-\psi_1-\hat\psi =0$ on $\partial B_L$, that is, $\psi-\psi_1-\hat\psi\in\zbHone[B_L]$. Then
\begin{align*}
\big|\langle \tilde F,\psi\rangle\big| =  \big|\langle F,\psi-\psi_1-\hat\psi\rangle\big| 
\le \|F\|_{H^{-1}(B_L)} \big\|\psi-\psi_1-\hat\psi\big\|_{\Hone[B_L]}
\le C\|F\|_{H^{-1}(B_L)} \|\psi\|_{\Hone[B_L]}.
\end{align*}
We conclude that $\big\|\tilde F\big\|_{H^{-1}(\wt B_L)} \le C\|F\|_{H^{-1}(B_L)}$.

		
By the Hahn-Banach theorem, we may extend $\tilde F$ to a functional
$F_1\in H^{1}(\bbR^2)'$ such that
\[
\|F_1\|_{H^{1}(\bbR^2)'}=\big\|\tilde F\big\|_{H^{-1}(\wt B_L)}
\le C\|F\|_{H^{-1}(B_L)}.
\]
By Lemma~\ref{lem:upml-whole}, there exists a unique $w\in H^1(\bbR^2)$ which satisfies
\begin{align}
&\mathscr{A}_{\bbR^2}(w,\psi)=\langle F_1,\psi\rangle	
    \quad	\forall\,\psi\in H^1(\bbR^2), \notag \\
&\|w\|_{H^1(\bbR^2)}\le	Ck\ln k\|F_1\|_{H^{1}(\bbR^2)'}
\le	Ck\ln k\|F\|_{H^{-1}(B_L)}.    \label{w-est}
\end{align}
Define $z= w-\tilde\phi$. Then \eqref{problem-tF} shows
$\mathscr{A}_{\wt B_L}(z,\psi) = \big\langle F_1,\psi\big\rangle -\big\langle\tilde{F},\psi\big\rangle =0$ for $\psi\in H_0^1(\wt B_L)$.
Therefore,
\[
\Cl z =0 \quad \hbox{in}\;\; \wt B_L. 
\]

Next we define $\wh B_{L}:= (-2L_1+2l_1, 2L_1 -2l_1)\times (-2L_2+2l_2, 2L_2 -2l_2)$, and let $\chi\in C_0^\infty(\bbR^2)$ be a cutoff function which satisfies $\chi\equiv 1$ in $\wh B_L$ and $\chi\equiv 0$ outside $\wt B_L$. We define $\tilde{z} =\chi z$ and extend it by zero to $\bbR^2\backslash\wt B_L$. Using \eqref{eq:pml-fundamental} and integration by part, we find that, for $\Bx\in B_L$,  
\begin{align*}
J(\Bx)z(\Bx) = \int_{\wt B_L} \Cl_{\By}\wt G(\By,\Bx) \,
J(\By)\tilde{z}(\By)\D\By 
= \int_{\wt B_L}  J(\By)\wt G(\By,\Bx) \,(\Cl\tilde{z})(\By)\D\By 
= \int_{\wt B_L\backslash\wh B_L} \wt G(\By,\Bx) \zeta(\By) \D\By,
\end{align*}
where $\zeta:= \nabla\cdot(\bbA\nabla\chi)\, z +2(\bbA\nabla\chi)\cdot\nabla z$ admits
\begin{align}\label{zeta-est} 
\NLtwo[\wt B_L]{\zeta}  \le C\NHone[\wt B_L]{z}
\le C\big(\NHone[\wt B_L]{w}+\|\phi\|_{\Hone[B_L]}\big)  .
\end{align}



Recall the identity $G(\tilde\By,\tilde\Bx) = G(\tilde\Bx,\tilde\By)$ and Lemma~\ref{lem:decay-stretchedG}. The assumption of the lemma shows $|\Bx-\By|>d-l>R$ with $d=\min\{d_1,d_2\}$ and $l=\max\{l_1,l_2\}$. We obtain
\begin{align*} 
\int_{\wt B_L\backslash\wh B_L}\int_{B_L} \big|\nabla^j_{\Bx} 
G(\tilde\By,\tilde\Bx)\big|^2 \D\Bx\D\By
\le\,& Ck^{2j} \int_{\wt B_L\backslash\wh B_L}\int_{B_L}(k|\Bx-\By|)^{-1}
e^{-\frac{1}{4}\sigma_0k|\Bx-\By|} \D\Bx\D\By \\
\le\,& Cdk^{2j-1}  \int_{d-l}^{\infty} e^{-\frac{1}{4}\sigma_0kr} \D r \\
\le\,& C d k^{2j-2}  e^{-\frac{1}{5}\sigma_0 kd},\quad j=0,1.
\end{align*}
By \eqref{zeta-est} and the identity $\wt G(\By,\Bx) = J(\Bx)G(\tilde\By,\tilde\Bx)$, we obtain
\begin{align*}
\NLtwov[B_L]{\nabla^jz}^2 
=\,&\int_{B_L}\bigg|\int_{\wt B_L\backslash\wh B_L} 
\nabla^j_{\Bx} G(\tilde\By,\tilde\Bx)
\,\zeta(\By) \D\By\bigg|^2 \D\Bx  \\
\le\,& \NHone[\wt B_L\backslash \wh B_L]{\zeta}^2 
\int_{\wt B_L\backslash\wh B_L}\int_{B_L} \big|\nabla^j_{\Bx} 
G(\tilde\By,\tilde\Bx)\big|^2 \D\Bx\D\By \\
\le\,& Cd k^{2j-2}  e^{-\frac{1}{5}\sigma_0 kd}
\big(\NHone[B_L]{w}^2 +\NHone[B_L]{\phi}^2\big),\quad j=0,1.
\end{align*}
We conclude that
\begin{align*}
\NHone[B_L]{\phi}^2 \le \big(1+Cd e^{-\frac{1}{5}\sigma_0 kd}\big) \NHone[B_L]{w}^2  
+ C d e^{-\frac{1}{5}\sigma_0 kd}\NHone[B_L]{\phi}^2.
\end{align*}
The proof is finished by using \eqref{w-est} and setting $\sigma_0d$ large enough such that $C d e^{-\frac{1}{5}\sigma_0 kd}<1/2$.
\end{proof}
 
\subsection{Well-posedness of \eqref{pml-source}}

We end this section by presenting the well-posedness of problem \eqref{pml-source}. It is a direct result of Theorem~\ref{thm:infsup-BL}. \vspace{1mm}

\begin{theorem}
Problem \eqref{pml-source} has a unique solution $\hat{u}\in\zbHone[B_L]$. Moreover, there exists a constant $C$ independent of $k$ such that
\[
\NHone[B_L]{\hat{u}} \le C\ln k \NLtwo[B_l]{f}.
\]
\end{theorem}
\begin{proof}
The existence and uniqueness of the solution come directly from Theorem~\ref{thm:infsup-BL}. To prove the stability,  we use \eqref{eq:infsup-BL} and find
\begin{align*}
\NHone[B_L]{\hat{u}} \le Ck\ln k \sup_{0\neq v\in H_0^1(B_L)}
\frac{|\mathscr{A}_{B_L}(\hat{u},v)|}{\|v\|_{H^1(B_L)}}
= Ck\ln k \sup_{0\neq v\in H_0^1(B_L)}
\frac{|(f,\Bar{v})_{B_l}|}{\|v\|_{H^1(B_L)}}
\le C\ln k \NLtwo[B_l]{f}.
\end{align*}
The proof is finished.
\end{proof}



%%%
